Likelihood-Free Overcomplete ICA and Applications in Causal Discovery

Causal discovery witnessed significant progress over the past decades. In particular, many recent causal discovery methods make use of independent, non-Gaussian noise to achieve identifiability of the causal models. Existence of hidden direct common causes, or confounders, generally makes causal discovery more difficult; whenever they are present, the corresponding causal discovery algorithms can be seen as extensions of overcomplete independent component analysis (OICA). However, existing OICA algorithms usually make strong parametric assumptions on the distribution of independent components, which may be violated on real data, leading to sub-optimal or even wrong solutions. In addition, existing OICA algorithms rely on the Expectation Maximization (EM) procedure that requires computationally expensive inference of the posterior distribution of independent components. To tackle these problems, we present a Likelihood-Free Overcomplete ICA algorithm (LFOICA) that estimates the mixing matrix directly by back-propagation without any explicit assumptions on the density function of independent components. Thanks to its computational efficiency, the proposed method makes a number of causal discovery procedures much more practically feasible. For illustrative purposes, we demonstrate the computational efficiency and efficacy of our method in two causal discovery tasks on both synthetic and real data.

==> v0/abstract.tex <==
Causal discovery enjoys significant progress over the past few years. Especially, many recent causal discovery methods make use of independent non-Gaussian noise to guarantee identifiability of the causal models. The corresponding causal discovery algorithms are extensions of over-complete independent component analysis (OICA). However, previous OICA algorithms make strong parametric assumptions on the distribution of independent components, which restricts the deployment of causal discovery algorithms on real data. In addition, the current OICA algorithms rely on the Expectation Maximization (EM) procedure that requires computationally expensive inference of the posterior distribution of independent components. To tackle these problems, we present an adversarial over-complete ICA algorithm that estimates the mixing matrix directly by back-propagation. We demonstrate the advantages of our method in two causal discovery tasks on both simulated and real data.

% Independent component analysis(ICA) and it's variants have been extensively used in many fields, such as blind source separation(BSS), unsupervised feature learning and causal discovery. However, standard ICA assumes that the number of components won't exceed that of observed mixtures, which makes it difficult to deal with over-complete cases(with more components than mixtures). Previous over-complete ICA algorithms make strong assumptions to the distribution of components, and have difficulties dealing with large number of components due to high computational complexity. To tackle these problems, we present an adversarial learning framework for over-complete ICA problem(AICA). We demonstrate that our method has advantages over previous method and further explore it's applications in two causal discovery problems.

==> v0/application.tex <==
\label{sec:Applications In Causal Discovery Of Time Series}
Here we explore the applications of the AOICA framework in causal discovery.  Two causal discovery problem are analyzed. One is estimating causal relation under measurement error. The other is estimating causal relation from down-sampled time-series.
\subsection{Causal discovery under measurement error}
Measurement error(i.g. noise caused by sensors) in the observed data can lead to inaccurate result of various causal discovery methods. \cite{Zhang2018CausalDW} proved the identifiability of linear, non-Gaussian causal model with measurement error, under some assumptions. Here we will apply AOICA framework to discover the causal relation in this problem.

Following \cite{Zhang2018CausalDW}, we use the linear model
\begin{equation}
    \tilde{\mathbf{X}}=\mathbf{B} \tilde{\mathbf{X}}+\tilde{\mathbf{E}}
\end{equation}
where $\tilde{\mathbf{X}}$ is the data generated by causal model without noise, $\mathbf{B}$ is the corresponding causal adjacency matrix, where $B_{ij}$ is the coefficient of the direct causal influence from $\tilde{X}_j$ to $\tilde{X}_i$. As we can see, $\tilde{\mathbf{X}}$ is actually a linear transformation of the error terms 
\begin{equation}
    \tilde{\mathbf{X}}=(\mathbf{I}-\mathbf{B})^{-1} \tilde{\mathbf{E}}
\end{equation}
Then, measurement error is added
\begin{align}
\label{equ:measurementerror}
    \notag \mathbf{X} = \tilde{\mathbf{X}} + \mathbf{E}&=(\mathbf{I}-\mathbf{B})^{-1} \tilde{\mathbf{E}} +\mathbf{E}\\
    &=\left[(\mathbf{I}-\mathbf{B})^{-1}\quad \mathbf{I}\right]\left[\begin{array}{c}
         \tilde{\mathbf{E}}\\
         \mathbf{E}
    \end{array}\right]
\end{align}
Where $\mathbf{X}$ is observed data, $\mathbf{E}$ is measurement error. Equation \ref{equ:measurementerror} has the same form as over-complete ICA, where $\left[(\mathbf{I}-\mathbf{B})^{-1}\quad \mathbf{I}\right]$ is the mixing matrix. So the AOICA framework can be applied to estimate $\mathbf{B}$.

\subsection{Causal discovery from down-sampled time series}
Granger causal analysis has been extensively applied in temporal causal discovery of time series. Time series $x_1$ is said to have Granger causal effect on another time series $x_2$ if and only if the past and current value of $x_1$ is helpful in predicting the future value of $x_2$ while it is not the case in the reverse side. Usually we use vector autoregressive(VAR) models to discover the Granger causal relations. We often assume that the VAR model serves as the true data generating process, which means the causal relation revealed by VAR model equals to the true causal frequency. However, the frequency of the data we measured is often lower than the true causal frequency(i.e. we often down sample data using sensors at a fixed frequency). This means we can not apply VAR model in the down-sampled data.


According to \cite{subsampled}, there are two typical down-sampling schemes to obtain low frequency data from original high frequency ones. One is called "subsampling": for every $k$ consecutive data points, one is kept and the others being dropped. Another is called "aggregating": it takes the average of $k$ consecutive and non-overlapping data points as the new observation. Here $k$ is called subsampling factor and aggregating factor respectively.


In this paper we use the same setting as in \cite{subsampled}. We assume the data in original causal frequency as a first order vector autoregressive process(VAR(1)). The graphical representation for this process is illustrated in Figure \ref{fig:originalcausalfreq}.
\begin{equation}
\label{equ:originalprocess}
    \mathbf{x}_t=\mathbf{A}\mathbf{x}_{t-1}+\mathbf{e}_t
\end{equation}
Where $\mathbf{x}_t$ is a $n$ dimensional vector at time step $t$. $\mathbf{A} \in \mathds{R}^{n\times n}$ is the transition matrix at true causal frequency, $\mathbf{e}_t \in \mathds{R}^{n}$ is noise at time step $t$. We will explore how to recover true causal relation(i.e. transition matrix $\mathbf{A}$) in both subsampling and aggregating scenarios with our adversarial framework under specific assumptions.
\begin{figure}[htbp]
\centering 
\subfigure[]{
\label{fig:originalcausalfreq}
\includegraphics[width=0.45\textwidth]{figures/originalprocess.eps}}
\subfigure[]{
\label{fig:subsamplingk}
\includegraphics[width=0.45\textwidth]{figures/subsampled.eps}}
\subfigure[]{
\label{fig:baselinesubsampled}
\includegraphics[width=0.45\textwidth]{figures/baseline_model.eps}}
\subfigure[]{
\label{fig:conditionalsubsampled}
\includegraphics[width=0.45\textwidth]{figures/conditional_model.eps}}
\caption{Graphical representation of (a) data generation process with original causal frequency (b) subsampled data generation proces with subsampling factor $k$ (c) AICA-baseline model for subsampled data with subsampling factor $k$ (d) AICA-conditional model for subsampled data with subsampling factor $k$.}
\end{figure}

\paragraph{Causal discovery from subsampled time series}
\label{sec:subsample}
We consider the following subsampling scheme\cite{subsampled} with subsampling factor $k$.
\begin{align} 
\label{equ:subsample}
\tilde{\mathbf{x}}_{t+1} &= \mathbf{x}_{1+tk} = \mathbf{Ax}_{1+tk-1}+\mathbf{e}_{1+tk} \notag \\
&= \mathbf{A}(\mathbf{Ax}_{1+tk-2}+\mathbf{e_{1+tk-1}})+\mathbf{e}_{1+tk}\notag \\
&=...\notag \\
&=\mathbf{A}^k\mathbf{\tilde{x}}_t+\sum_{l=0}^{k-1}\mathbf{A}^l\mathbf{e}_{1+tk-l}
\end{align}
Where $\tilde{\mathbf{x}}_{t}$ is subsampled data. In other words, we can't observe the original data $\mathbf{x}_t$ directly. Instead, we only have access to subsampled data $\tilde{\mathbf{x}}_{t}$. And we wish to estimate transition matrix $\mathbf{A}$ at original causal frequency from these subsampled data. As we can seen from Equation \ref{equ:subsample}, for different time step in $\mathbf{\tilde{x}}$, the corresponding noise(i.e. the second term in the right hand of Equation \ref{equ:subsample}) are independent. Thus we can express Equation \ref{equ:subsample} as following
\begin{align}
\label{equ:subsample2}
    \tilde{\mathbf{x}}_{t+1} &= \mathbf{A}^k\mathbf{\tilde{x}}_t+\mathbf{L\tilde{e}}_{t+1}
\end{align}
where 
\begin{align}
    \mathbf{L}&= [\mathbf{I, A, A^2, ..., A^{k-1}}]\notag\\
    \mathbf{\tilde{e}} &= (\mathbf{e}_{1+tk-0}^\top, \mathbf{e}_{1+tk-1}^\top, ..., \mathbf{e}_{1+tk-(k-1)}^\top)^\top \notag
\end{align}
Equation \ref{equ:subsample2} can be regarded as a VAR(1) model with noise $\mathbf{L\tilde{e}}$ that is independent among different time steps as well. Graphical representation of this subsampled data is illustrated in Figure \ref{fig:subsamplingk}. 
% \begin{figure}[htbp]
% \centering 
% \includegraphics[width=0.45\textwidth]{figures/subsampled.eps}
% \caption{Graphical representation of subsampled data with sampling factor $k$}
% \label{fig:subsampledprocess}
% \end{figure}


Basically, \cite{subsampled} made use of second-order statistical information(i.e. autocovariances) to first estimate $\mathbf{A}^k$ and get rid of the contribution of the first term in Equation \ref{equ:subsample2} to give
\begin{equation}
\label{equ:icasubsampled}
    \Delta{\tilde{\mathbf{x}}}_{t+1} = \mathbf{L\tilde{e}}_{t+1}
\end{equation}
where $\Delta{\tilde{\mathbf{x}}}_{t+1}=\tilde{\mathbf{x}}_{t+1}-\mathbf{A}^k\mathbf{\tilde{x}}_t$. It is illustrated in Figure \ref{fig:baselinesubsampled}. It can be easily seen that Equation \ref{equ:icasubsampled} has the same over-complete ICA form as Equation \ref{equ:ica} when subsampling factor $k>1$. The adversarial over-complete ICA fromework, in which the generator $G_{\hat{\mathbf{A}}}(\cdot)$ conrrespoding to $\mathbf{L}\tilde{\mathbf{e}}_{t+1}$, can be applied to learn the transition matrix $\mathbf{A}$ at true causal frequency. We call this model of first estimating $\mathbf{A}^k$ then using adversarial ICA framework as "AICA-baseline model" for subsampled data. 


However, the estimation to $\mathbf{A}^k$ may be inaccurate as the number of dimensions grows larger. This will lead to incorrect calculation of $\Delta\tilde{\mathbf{x}}_t$. As a consequence, the estimation to $\mathbf{A}$ will be incorrect as well. \cite{cgan} uses training labels as additional inputs to both generator and discriminator, which can be seen as a conditional model. Motivated by this, we modify the AICA-baseline model to have conditional input. We call this modified model as AICA-conditional.This model  combines both the idea of traditional maximum likelihood estimation and the idea of GAN-style learning, to learn both the relation between $\mathbf{\tilde{e}}_t$ and $\mathbf{\tilde{x}}_t$(i.e. $\mathbf{L}$) and the relation between $\mathbf{\tilde{x}}_t$ and  $\mathbf{\tilde{x}}_{t+1}$(i.e. $\mathbf{A}^k$) jointly. Thus, the estimation of $\mathbf{A}^k$ is avoided. See Algorithm \ref{alg:conditional adversarial learning} for detailed description and Figure \ref{fig:conditionalsubsampled} for graphical representation for this conditional model.% Suppose we have $N$ subsampled data $(\mathbf{\tilde{x}}_1, \mathbf{\tilde{x}}_2, ..., \mathbf{\tilde{x}}_N)$. We first sample $\mathbf{\tilde{x}}_t$ from the subsampled data as conditions. Then we take $\mathbf{\tilde{x}}_{t+1}$ as target data. The generator takes both non-Gaussian noise and conditions as inputs and generate $\mathbf{\hat{\tilde{x}}}_{t+1}$. $\mathbf{\hat{\tilde{x}}}_{t+1}$ at different time steps can be regarded as independent by condition on $\mathbf{\tilde{x}}_{t}$. Then MMD can be calculated as the distance between the conditional distributions $p(\mathbf{\tilde{x}}_{t+1}|\mathbf{\tilde{x}}_{t})$ and $p(\mathbf{\hat{\tilde{x}}}_{t+1}|\mathbf{\tilde{x}}_{t})$. Finally optimization method is used to minimize MMD. 

% \begin{figure}[htbp]
% \centering 
% \subfigure[Baseline model]{
% \label{fig:baselinesubsampled}
% \includegraphics[width=0.45\textwidth]{figures/baseline_model.eps}}
% \subfigure[Conditional model]{
% \label{fig:conditionalsubsampled}
% \includegraphics[width=0.45\textwidth]{figures/conditional_model.eps}}
% \caption{Graphical representations of two models for subsampled data with sampling factor $k$}
% \end{figure}

\begin{algorithm}[t]
\caption{Conditional Adversarial Learning For Subsampled Data} 
\label{alg:conditional adversarial learning}
\begin{algorithmic}[1]
    \State Get a minibatch of samples $\tilde{\mathbf{x}}_t$ from $(\tilde{\mathbf{x}}_1, \tilde{\mathbf{x}}_2, ..., \tilde{\mathbf{x}}_N)$ as conditions
    \State For each $\tilde{\mathbf{x}}_t$ in the minibatch obtained in step 1, take the corresponding  data of next time step $\tilde{\mathbf{x}}_{t+1}$ from $(\tilde{\mathbf{x}}_1, \tilde{\mathbf{x}}_2, ..., \tilde{\mathbf{x}}_N)$ as targets
    \State Get a minibatch of samples from $p(\mathbf{z})$ 
    \State Mapping $\mathbf{z}$ using parameterized $f_\theta(\cdot)$, get non-Gaussian noise $\hat{\mathbf{s}}$
    \State Generator takes non-Gaussian noise $\hat{\mathbf{s}}$ and conditions $\tilde{\mathbf{x}}_t$ as inputs and generate target data $\mathbf{\hat{\tilde{x}}}_{t+1} = \mathbf{A}^k \tilde{\mathbf{x}}_t + \hat{\mathbf{s}}$
    \State Calculate distribution distance between $p(\hat{\tilde{\mathbf{x}}}_{t+1}|\tilde{\mathbf{x}}_{t})$ and $p(\tilde{\mathbf{x}}_{t+1}|\tilde{\mathbf{x}}_{t})$ using MMD 
    \State Using optimization algorithms such as SGD to update $\hat{\mathbf{A}}$ and $\theta$ by minimizing MMD
    \State Repeat step 1 to step 7 until max iterations reached
\end{algorithmic}
\end{algorithm}


It has been proved in \cite{subsampled} that besides the two assumptions mentioned in section \ref{sec:AOICA}, if we further assume that the $n$ components of $\mathbf{e}_{t}$ in Equation \ref{equ:originalprocess} have different distributions, the permutation and scaling indeterminacies can be eliminated with only sign indeterminacy left.

% The AICA-conditional model achieves desirable result on subsampled time series data, which is demonstrated in Section \ref{sec:subsampledtotal}.

\paragraph{Causal discovery from aggregated time series}
\label{sec:aggregate}
We consider the following aggregating scheme\cite{aggregated} with aggregating factor $k$.
\begin{align}
\label{equ:aggregate}
\tilde{\mathbf{x}}_{t}=&\frac{1}{k} \sum_{i=1}^{k} \mathbf{x}_{i+(t-1) k} \notag \\
=&\frac{1}{k} \sum_{i=1}^k \left (\mathbf{A}^{k} \mathbf{x}_{i+(t-2) k}+\sum_{l=0}^{k-1} \mathbf{A}^{l}\mathbf{e}_{i+(t-1) k-l}\right)\notag \\
=&\frac{\mathbf{A}^{k}}{k} \sum_{i=1}^{k} \mathbf{x}_{i+(t-2) k}+\frac{1}{k} \sum_{i=1}^{k}\left(\sum_{l=0}^{k-1} \mathbf{A}^{l} \mathbf{e}_{i+(t-1) k-l}\right)\notag \\
=&\mathbf{A}^{k} \tilde{\mathbf{x}}_{t-1}+\frac{1}{k}\left(\sum_{m=0}^{k-1}\left(\sum_{n=0}^{m} \mathbf{A}^{n}\right) \mathbf{e}_{t k-m}+\sum_{m=1}^{k-1}\left(\sum_{n=m}^{k-1} \mathbf{A}^{n}\right) \mathbf{e}_{(t-1) k-m+1} \right)
\end{align}
Where $\tilde{\mathbf{x}}_t$ is aggregated data which can be observed directly. For notation simplicity, \cite{aggregated} express Equation \ref{equ:aggregate} as follows
\begin{align}
\label{equ:notationsim}
\tilde{\mathbf{x}}_{t} &=\mathbf{A}^{k} \tilde{\mathbf{x}}_{t-1}+\tilde{\mathbf{e}}_{t} \notag\\ &=\mathbf{A}^{k} \tilde{\mathbf{x}}_{t-1}+\mathbf{M}_{0} \mathbf{\epsilon}_{t}+\mathbf{M}_{1} \mathbf{\epsilon}_{t-1} 
\end{align}
Where 
\begin{align}
\mathbf{\epsilon}_{t}=&\frac{1}{k}\left[\mathbf{e}_{t k}, \mathbf{e}_{t k-1}, \ldots, \mathbf{e}_{(t-1) k+1}\right]^{\top}\notag \\
\mathbf{M}_0=&\left[\mathbf{I}, \mathbf{I}+\mathbf{A}, \ldots, \sum_{n=0}^{k-1} \mathbf{A}^{n} \right]\notag \\
\mathbf{M}_{1}=&\left[\sum_{n=1}^{k-1} \mathbf{A}^{n}, \ldots, \mathbf{A}^{k-1}, \mathbf{0}\right]\notag
\end{align}
It's a vector autoregressive moving average(VARMA) with one autoregressive term and two moving-average terms. Different from Equation \ref{equ:subsample2} in subsampling scenarios, the noise item in Equation \ref{equ:notationsim} is dependent at different time steps. For example, the noise item for $\tilde{\mathbf{x}}_{t} $ is $\mathbf{M}_{0} \mathbf{\epsilon}_{t}+\mathbf{M}_{1} \mathbf{\epsilon}_{t-1}$ and the noise item for $\tilde{\mathbf{x}}_{t-1}$ is $\mathbf{M}_{0} \mathbf{\epsilon}_{t-1}+\mathbf{M}_{1} \mathbf{\epsilon}_{t}$, which means there exists overlap between noise items of two consecutive time steps. Graphical representation for aggregated data is illustrated in Figure \ref{fig:aggregatedprocess}.
\begin{figure}[htbp]
    \centering
    \subfigure[]{
    \label{fig:aggregatedprocess}
    \includegraphics[width=0.45\textwidth]{figures/aggregated.eps}}
    \subfigure[]{
    \label{fig:conditionalaggregated}
    \includegraphics[width=0.45\textwidth]{figures/conditional_model_aggregated.eps}}
    \subfigure[]{
        \label{fig:pieces}
    \includegraphics[width=0.45\textwidth]{figures/conditional_model_aggregated_piece.eps}}
    \caption{Graphical representation of aggregated data with aggregating factor $k$}
\end{figure}


Things become more complicated in this case. We can no longer decouple the relation between different time steps as we did in baseline model of subsampling scenario. Conditional model can't be applied directly to this problem because $\mathbf{\tilde{x}}_{t+1}$ are not independent even if conditioned on previous data point $\mathbf{\tilde{x}}_{t}$(for example $\mathbf{\tilde{x}}_{t+1}$ and $\mathbf{\tilde{x}}_{t}$ are still connected through $\mathbf{\epsilon}_t$). This is illustrated in Figure \ref{fig:conditionalaggregated}.
% \begin{figure}[htbp]
%     \centering
%     \subfigure[]{
%     \label{fig:conditionalaggregated}
%     \includegraphics[width=0.45\textwidth]{figures/conditional_model_aggregated.eps}}
%     \subfigure[]{
%     }
%     \caption{Naive conditional model for aggregated data with aggregating factor $k$}
% \end{figure}


State Space GAN(SSGAN) is proposed in \cite{graphicalGAN} as an instance of graphical GAN to learn recognition model and generation model jointly and apply this model to visual datasets with temporal relations such as Moving MNIST \cite{movingmnist}. Inspired by SSGAN and it's application to Moving MNIST, we process our aggregated time series data to mimic the special traits of Moving MNIST. Moving MNIST contains 10,000 sequences each of length 20 showing 2 digits moving in a 64 x 64 frame. In this dataset, each data point is a time sequence. Thus, we divide the aggregated time series into pieces of equal length without overlapping. Figure \ref{fig:pieces} is an illustration of one such piece with length 4.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/conditional_model_aggregated_piece.eps}
%     \caption{Graphical illustration of divided piece of aggregated time series with length 4}
%     \label{fig:pieces}
% \end{figure}
\begin{algorithm}[htbp]
\caption{Conditional Adversarial Learning For Aggregated Data} 
\label{alg:conditional adversarial learning_aggregated}
\begin{algorithmic}[1]
    \State Divide the aggregated time series into pieces of length $l$. These pieces form a minibatch
    \State Take the first element $\tilde{\mathbf{x}}_{t}$ as condition and the other elements $\tilde{\mathbf{x}}_{t+1}, \tilde{\mathbf{x}}_{t+2}, ..., \tilde{\mathbf{x}}_{t+n-1}$ as targets
    \State Get a minibatch of samples from $p(\mathbf{z})$
    \State Mapping $\mathbf{z}$ using parameterized $f_\theta(\cdot)$, get non-Gaussian noise $\hat{\mathbf{\epsilon}}_t, \hat{\mathbf{\epsilon}}_{t+1}, ..., \hat{\mathbf{\epsilon}}_{t+l-1}$. All the noises are i.i.d.
    \State Generator takes non-Gaussian noise $\hat{\mathbf{\epsilon}}_t$, $\hat{\mathbf{\epsilon}}_{t+1}$ and conditions $\tilde{\mathbf{x}}_t$ as inputs and generate target data $\hat{\mathbf{\tilde{x}}}_{t+1}$ using Equation \ref{equ:notationsim}, $\hat{\tilde{\mathbf{x}}}_{t+2}, \hat{\tilde{\mathbf{x}}}_{t+3}, ..., \hat{\tilde{\mathbf{x}}}_{t+n-1}$ are generated in the same way
    \State Calculate distribution distance between $p(\hat{\tilde{\mathbf{x}}}_{t+1}, \hat{\tilde{\mathbf{x}}}_{t+2}, ..., \hat{\tilde{\mathbf{x}}}_{t+n-1}|\tilde{\mathbf{x}}_{t})$ and $p(\tilde{\mathbf{x}}_{t+1}, \tilde{\mathbf{x}}_{t+2}, ..., \tilde{\mathbf{x}}_{t+n-1}|\tilde{\mathbf{x}}_{t})$ using MMD 
    \State Using optimization algorithms such as SGD to update $\hat{\mathbf{A}}$ and $\theta$ by minimizing MMD
    \State Repeat step 1 to step 7 until max iterations reached
\end{algorithmic}
\end{algorithm}


We can consider our aggregated data as composed of many such pieces without overlapping. In SSGAN, generation model and inference(recognition) model is learned jointly by matching the joint distribution $q(\mathbf{\epsilon}_t, \mathbf{\epsilon}_{t+1}, \mathbf{\epsilon}_{t+2}, \mathbf{\epsilon}_{t+3}, \tilde{\mathbf{x}}_{t+1}, \tilde{\mathbf{x}}_{t+2}, \tilde{\mathbf{x}}_{t+3})$ and $p(\mathbf{\epsilon}_t, \mathbf{\epsilon}_{t+1}, \mathbf{\epsilon}_{t+2}, \mathbf{\epsilon}_{t+3}, \tilde{\mathbf{x}}_{t+1}, \tilde{\mathbf{x}}_{t+2}, \tilde{\mathbf{x}}_{t+3})$, where $q$ and $q$ represent distributions generated by recognition model and generation model respectively.While in this problem, it's unnecessary to do inference because we don't care latent variables $\mathbf{\epsilon}$. So we simply match $q(\tilde{\mathbf{x}}_{t+1}, \tilde{\mathbf{x}}_{t+2}, \tilde{\mathbf{x}}_{t+3}|\tilde{\mathbf{x}}_{t})$ and $p(\tilde{\mathbf{x}}_{t+1}, \tilde{\mathbf{x}}_{t+2}, \tilde{\mathbf{x}}_{t+3}|\tilde{\mathbf{x}}_{t})$ based on the idea of conditional GAN \cite{cgan}. As the pieces are non-overlapping(here non-overlapping means each variable $\tilde{\mathbf{x}}_{t}$, including the condition variable, will only appear in one piece of data), the dependence issue is avoided because all the pieces can be regarded as independent. It's obvious that longer pieces are better because they model longer relations. However, in practice the number of observed data points is limited, which means the total length of aggregated time series is limited. Longer pieces will lead to smaller number of pieces, which means the batch size is smaller. And small batch size will lead to inaccurate result when calculating MMD\cite{gmmn}. There is a trade off between the length of each piece and the number of pieces. The effect of different length of piece is compared in Section \ref{sec:aggregatedtotal}. We call this method as AICA-divided. Detailed description is illustrated in Algorithm \ref{alg:conditional adversarial learning_aggregated}.

==> v0/experiment.tex <==
In this section, we first conduct empirical studies of the adversarial learning framework in over-complete scenario using synthetic data.Then we apply AICA framework to down-sampled time series data in both subsampled and aggregated scenarios on synthetic and real data to show their effectiveness of estimating causal relation. We also explore the application of AICA in causal discovery with measurement error on synthetic data.
\subsection{Recovering mixing matrix in over-complete scenario}
In this section, we compare the result of our adversarial ICA algorithm with that of several well-know n algorithm in over-complete scenario. The data is synthetic. Since the identifiability of the over-complete ICA model requires non-Gaussian distribution for all the independent components, we use Gaussian-mixtures with two Gaussians for each independent component. Each Gaussian has zero mean to make the Gaussian-mixture super-Gaussian. According to \cite{identifiabilityofica}, the mixting matrix can be estimated up to the permutation and scaling indeterminacies(including the sign indeterminacy) of the columns. We may want to eliminate these indetermincies for comparison purpose. To eliminate the permutation indeterminacy, the non-Gaussian distribution for each component is made not only independent, but also different. We use different mixing rate for each independent component to make the distributions different. With different distributions for each component, it is convenient to permute the columns to the same order for all the algorithms. In order to eliminate the scaling indeterminacy for comparison purpose, we normalize each column of the mixing matrix according to the ratio of the recovered components' variance to the true independent components' variance(this is achievable because the data is synthetic). With the permutation and scaling indeterminacy eliminated, we can conveniently compare the mixing matrix obtained by different algorithms. 

Table \ref{table:overcompleteica} shows the results of several over-complete ICA algorithms. In the table, RICA represents reconstruction ICA\cite{le2011ica}, MFICA\_Gauss, MFICA\_MOG, MFICA\_biGauss represents mean-field ICA\cite{hojen2002mean} with the prior distribution of independent components set as Gaussian distribution, mixture of Gaussian distribution and biGaussian(sum of two Gaussians) distribution respectively. AICA represents our adversarial learning ICA. Here $m$ is the number of observed mixtures, $n$ is the number of independent components. For each algorithm, we conduct experiment in 4 cases([m=2 n=4], [m=3 n=6], [m=4 n=8] and [m=5 n=10]). Each experiment is repeated 10 times and the results are averaged. All the estimated mixing matrices are processed as said above to eliminate the permutation and scaling indeterminacy. As we can see from the table, our adversarial learning ICA framework achieves best result compared with the others.

To further demonstrate the ability of our adversarial ICA framework to recover the original independent components, we draw the scatter plot of the first two recovered components in the case where the number of mixtures $m=2$ and the number of components $n=4$ in Figure \ref{fig:subsample_fake_noise}. The scatter plot of the first two original components is also shown in Figure \ref{fig:subsample_true_noise} for comparison. As we can see from the figures, the two components with two different super-Gaussian distributions are well-recovered.
\begin{figure}[htbp]
\centering 
\subfigure[Recovered components]{
\label{fig:subsample_fake_noise}
\includegraphics[width=0.45\textwidth]{figures/subsample_fake_noise.png}}
\subfigure[Original components]{
\label{fig:subsample_true_noise}
\includegraphics[width=0.45\textwidth]{figures/subsample_true_noise.png}}
\end{figure}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{MSE of the recovered mixing matrix by different methods on simulated data in over-complete ICA scenario.}
\begin{tabular}{@{}ccccc@{}}
\toprule
Methods        & m=2, n=4         & m=3, n=6         & m=4, n=8         & m=5, n=10        \\ \midrule
RICA           & 2.26e-2          & 1.54e-2          & 9.03e-3          & 7.54e-3          \\
MFICA\_Gauss   & 4.54e-2          & 2.45e-2          & 4.21e-2          & 3.18e-2          \\
MFICA\_MOG     & 2.38e-2          & 9.17e-3          & 2.43e-2          & 1.04e-2          \\
MFICA\_biGauss & 1.82e-2          & 6.56e-3          & 1.21e-2          & 1.34e-2          \\
AICA           & \textbf{4.61e-3} & \textbf{5.95e-3} & \textbf{6.96e-3} & \textbf{5.92e-3} \\ \bottomrule
\end{tabular}
 
\label{table:overcompleteica}
\end{table}
\subsection{Recovering causal relation from subsampled time series data}
\label{sec:subsampledtotal}
In this section, we will apply the adversarial ICA framework to recover causal relation from both synthetic data and real data in subsampling scenario.
\subsubsection{Synthetic data}
\label{sec:subsampledsynthetic}
Following \cite{subsampled}, we generate the time series data at the original causal frequency using VAR(1) model described by Equation \ref{equ:originalprocess}. The matrix $\mathbf{A}$ is generated randomly with it's diagonal elements sampled from uniform distribution $U(0.5, 1)$ and it's non-diagonal elements sampled from uniform distribution $U(0, 0.5)$. This is based on the fact that in most cases the inter-channel temporal causal relation is stronger than that of cross-channel. To make the noise non-Gaussian distributed, we model the distribution for each channel of the noise as Gaussian mixtures with two components: for each channel, component 1 is distrubuted as $N(0, 0.1)$ and component 2 is distributed as $N(0, 4)$. Since one of the assumptions for the model to be identifiable with the permutation and scaling indeterminacies eliminated is that different channels of the noise have different non-Gaussian distributions, we use different mixing rates to mix the two Gaussian components for different channels. Low-resolution observations were obtained by subsampling the high-resolution data using subsampling factor $k$. We set the number of dimensions $n=2, 5$, subsampling factor $k=2, 3, 4, 5$ and sample size $T=100, 300, 1000, 3000$ for subsampled data. We repeat each experiment for 10 times and averaging the results.


Table \ref{table:subsampledcompare_n_2_1} and  Table \ref{table:subsampledcompare_n_5_1} show the mean square error (MSE) of the estimated transition matrix $\mathbf{A}$ when number of dimensions $n=2$ and $n=3$ respectively in subsampling scenario. For each case, we conduct experiments when the subsampling factor $k=2,3,4,5$ and length of data $T=100, 300$. As one can see from Table \ref{table:subsampledcompare_n_2_1}, in low dimensional cases($n=2$ here), AICA-conditional model achieves comparable result as NG-EM and NG-MF in \cite{subsampled}. NG-EM has better performance when the number of data points is small($T=100$) because the MMD distance measure we use in AICA may be inaccurate with small number of samples. When the number of data points is larger($T=300$), AICA obtains best results. NG-EM and NG-MF have difficulties dealing with cases where the number of data dimension $n$ is larger, while our AICA-baseline model and AICA-conditional model are able to achieve reasonable results in this case, which can be seen from Table \ref{table:subsampledcompare_n_5_1} when $n=5$. 
\begin{table}[]
\centering
\caption{MSE of the recovered transition matrix by different methods on simulated data in subsampling scenario.}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{3}{*}{Methods} & \multicolumn{8}{c}{n=2}                                                                                                                                                    \\ \cmidrule(l){2-9} 
                         & \multicolumn{4}{c|}{T=100}                                                                     & \multicolumn{4}{c}{T=300}                                                 \\ \cmidrule(l){2-9} 
                         & k=2              & k=3              & k=4              & \multicolumn{1}{c|}{k=5}              & k=2              & k=3              & k=4              & k=5              \\ \midrule
AICA-baseline            & 7.03e-3          & 8.33e-3          & 1.44e-2          & \multicolumn{1}{c|}{4.37e-2}          & 1.67e-3          & 7.02e-3          & 8.27e-3          & 1.00e-2          \\ \midrule
AICA-conditional         & 7.25e-3          & 7.88e-3          & \textbf{8.45e-3} & \multicolumn{1}{c|}{\textbf{9.00e-3}} & \textbf{1.12e-3} & \textbf{3.87e-3} & \textbf{4.07e-3} & \textbf{6.23e-3} \\ \midrule
NG-EM                    & \textbf{6.50e-3} & \textbf{7.32e-3} & 1.02e-2          & \multicolumn{1}{c|}{1.04e-2}          & 7.24e-3          & 9.11e-3          & 9.54e-3          & 9.98e-3          \\ \midrule
NG-MF                    & 9.09e-3          & 9.89e-3          & 1.24e-2          & 2.19e-2                               & 8.46e-3          & 8.76e-3          & 1.01e-2          & 2.20e-2          \\ \bottomrule
\end{tabular}
    
\label{table:subsampledcompare_n_2_1}
\end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \multirow{3}{*}{Methods} & \multicolumn{8}{c}{n=2}                                                                            \\ \cmidrule(l){2-9} 
%                          & \multicolumn{4}{c|}{T=1000}                                & \multicolumn{4}{c}{T=3000}            \\ \cmidrule(l){2-9} 
%                          & k=2     & k=3     & k=4     & \multicolumn{1}{c|}{k=5}     & k=2     & k=3     & k=4     & k=5     \\ \midrule
% Baseline model           & 6.76e-4 & 7.95e-5 & 4.20e-4 & \multicolumn{1}{c|}{1.11e-3} & 8.22e-5 & 1.38e-4 & 6.58e-5 & 2.72e-4 \\ \midrule
% Conditional model        & 1.06e-3 & 2.94e-4 & 3.88e-4 & \multicolumn{1}{c|}{9.54e-4} & 2.28e-4 & 1.68e-4 & 1.90e-4 & 9.60e-4 \\ \midrule
% Other methods            & -       & -       & -       & \multicolumn{1}{c|}{-}       & -       & -       & -       & -       \\ \bottomrule
% \end{tabular}
%     
% \caption{MSE of the recovered causal relation by different methods on simulated data in subsampling scenario. The results are shown for subsampling factors$(k=2, 3, 4, 5)$, length of data $(T=1000, 3000)$ and number of dimensions $n=5$. Here \textit{Other methods} includes methods NG-EM, NG-MF and G-EM proposed in \cite{subsampled}, method BFL proposed in \cite{boot1967further} and method SW proposed in \cite{stram1986methodological}.}
% \label{table:subsampledcompare_n_2_2}
% \end{table}


% Table \ref{table:subsampledcompare_n_5_1} and Table \ref{table:subsampledcompare_n_5_2} shows the mean square error (MSE) of the estimated parameters $\mathbf{A}$ when number of dimensions $n=5$ in subsampling scenario. As one can see from Table \ref{table:subsampledcompare_n_5_1} and Table \ref{table:subsampledcompare_n_5_2}, although both baseline model and condition model are desirable enough to recover the original causal relation $\mathbf{A}$, the conditional model obtains better result that that of baseline model. One instance of original causal relation $\mathbf{A}$ and the estimated counterpart is recorded as follows, whose MSE is $5.5\times 10^{-3}$. It shows that $\tilde{\mathbf{A}}$ is very close to $\mathbf{A}$ under this MSE.
% \begin{equation*}
% \mathbf{A}=
% \left[
% \begin{array}{ccccc}
%      0.78 & 0.02 & 0.05 & 0.03 & 0.06 \\
%      0.18 & 0.89 & 0 & 0.05 & -0.03 \\
%      0.08 & 0.01 & 0.36 & 0 & -0.04 \\
%      0 & 0 & 0.11 & 0.79 & -0.03 \\
%      0 & 0.01 & 0.01 & 0.02 & 0.66
% \end{array}
% \right]
% , \tilde{\mathbf{A}}=
% \left[
% \begin{array}{ccccc}
%     0.7684 &  0.0137&  0.1033&  0.0046&  0.0541 \\
%     0.1734&  0.8847&  0.0327&  0.0248& -0.0259 \\
%     0.0959& -0.0008&  0.2999&  0.0019& -0.0395 \\
%     0.0120& -0.0076&  0.0816&  0.8054& -0.0332 \\
%     -0.0005& -0.0257& -0.3104&  0.2003&  0.7156 \\
% \end{array}
% \right]
% \end{equation*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{MSE of the recovered transition matrix  by different methods on simulated data in subsampling scenario.}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{3}{*}{Methods} & \multicolumn{8}{c}{n=5}                                                                                                                                                    \\ \cmidrule(l){2-9} 
                         & \multicolumn{4}{c|}{T=100}                                                                     & \multicolumn{4}{c}{T=300}                                                 \\ \cmidrule(l){2-9} 
                         & k=2              & k=3              & k=4              & \multicolumn{1}{c|}{k=5}              & k=2              & k=3              & k=4              & k=5              \\ \midrule
AICA-baseline            & 8.12e-3          & 8.96e-3          & 2.10e-2          & \multicolumn{1}{c|}{4.65e-2}          & 4.18e-3          & 7.56e-3          & 8.90e-3          & 1.75e-2          \\ \midrule
AICA-conditional         & \textbf{7.84e-3} & \textbf{8.27e-3} & \textbf{8.84e-3} & \multicolumn{1}{c|}{\textbf{9.36e-3}} & \textbf{1.07e-3} & \textbf{5.40e-3} & \textbf{5.31e-3} & \textbf{7.51e-3} \\ \midrule
NG-EM                    & 1.50e-2          & 2.32e-2          & 2.02e-2          & \multicolumn{1}{c|}{3.04e-2}          & 1.24e-2          & 2.11e-2          & 2.54e-2          & 2.98e-2          \\ \midrule
NG-MF                    & 3.09e-2          & 3.89e-2          & 3.24e-2          & \multicolumn{1}{c|}{4.19e-2}          & 2.46e-2          & 3.76e-2          & 3.01e-2          & 4.20e-2          \\ \bottomrule
\end{tabular}
    
\label{table:subsampledcompare_n_5_1}
\end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
% \multirow{3}{*}{Methods} & \multicolumn{8}{c}{n=5}                                                                            \\ \cmidrule(l){2-9} 
%                          & \multicolumn{4}{c|}{T=1000}                                & \multicolumn{4}{c}{T=3000}            \\ \cmidrule(l){2-9} 
%                          & k=2     & k=3     & k=4     & \multicolumn{1}{c|}{k=5}     & k=2     & k=3     & k=4     & k=5     \\ \midrule
% Baseline model           & 5.42e-3 & 4.74e-3 & 4.11e-3 & \multicolumn{1}{c|}{3.25e-3} & 4.38e-3 & 6.78e-4 & 1.66e-3 & 5.33e-4 \\ \midrule
% Conditional model        & 5.00e-4 & 1.73e-3 & 4.08e-3 & \multicolumn{1}{c|}{3.94e-3} & 1.89e-4 & 2e-4    & 3.77e-4 & 1.17e-4 \\ \midrule
% Other methods            & -       & -       & -       & \multicolumn{1}{c|}{-}       & -       & -       & -       & -       \\ \bottomrule
% \end{tabular}
%     
% \caption{MSE of the recovered causal relation by different methods on simulated data in subsampling scenario. The results are shown for subsampling factors$(k=2, 3, 4, 5)$, length of data $(T=1000, 3000)$ and number of dimensions $n=5$.}
% \label{table:subsampledcompare_n_5_2}
% \end{table}
\subsubsection{Real data}
\label{sec:subsampledrealdata}
Besides synthetic data, we conduct experiments on real data as well. Here we use Temperature Ozone data\cite{JMLR:v17:14-518}, which can be downloaded from \href{https://webdav.tuebingen.mpg.de/cause-effect/}{Database with cause-effect pairs}. Temperature Ozone data corresponds to 49th, 50th and 51st causal-effect pairs in the database. The 3 temperature ozone pairs are taken at 3 different place(Lausanne, Chaumont and Davos-See in Switzerland respectively) in year 2009. Each pair of data contains two variables, ozone and temperature with the ground true causal direction temperature $\longrightarrow$ ozone. 


To demonstrate the result when $n=2$, we use 50th pair as in \cite{subsampled}. The optimal subsampling factor $k$ can be determined using the method of cross-validation on the log-likelihood of the models. Here we use $k=2$ according to \cite{subsampled}. The estimated transition matrix $\mathbf{A}=\bigl[ \begin{smallmatrix}0.9310 & 0.1295 \\  -0.0017 & 0.9996\end{smallmatrix}\bigr]$, from which we can clearly find the causal direction from temperature to ozone.


As is mentioned in Section \ref{sec:subsampledsynthetic}, one of the main advantages of our conditional model over that proposed in \cite{subsampled} is that our model can deal with cases when the dimension of data is larger. Here we will demonstrate the result when $n=6$. Since each of the 3 data pairs contains two variables, we simply concatenate the 3 pairs together to a new dataset containing 6 variables($x_1, x_2,..., x_6$). The corresponding ground truth causal relation is $x_2 \longrightarrow x_1, x_4 \longrightarrow x_3, x_6 \longrightarrow x_5$, which is demonstrated graphically in Figure \ref{fig:Ground truth causal relation}. Similarly, we use $k=2$ according to cross-validation on the log-likelihood of the models\cite{subsampled}. The estimated transition matrix is
\begin{equation*}
    \mathbf{A} = \left[
    \begin{array}{cccccc}
                           0.8717&  0.4091& -0.0126& -0.0140&  0.0065& -0.0586\\
                           0.0180&  0.7093& -0.0224&  0.0866&  0.0039&  0.0972\\
                           0.0365& -0.0008&  0.8587&  0.2427&  0.0626&  0.0160\\
                          -0.0233&  0.0581&  0.0323&  0.6447& -0.0108&  0.0840\\
                           0.0188&  0.0336&  0.0774& -0.0552&  0.8553& -0.0722\\
                          -0.0338&  0.0730&  0.0245&  0.0718& -0.0013&  0.5782
    \end{array}\right]
\end{equation*}
The corresponding causal diagram is plotted in Figure \ref{fig:Causal relation of conditional model}. We further plot the causal diagram obtained by PC algorithm\cite{spirtes2000causation} and LiNGAM algorithm\cite{shimizu2006linear} in Figure \ref{fig:Causal relation of PC} and \ref{fig:Causal relation of LiNGAM}. As one can see from the figures, the only mistake of the causal diagram obtained by our method is the absence of arrow from $x_6$ to $x_5$ while PC algorithm and LiNGAM algorithm make other mistakes besides the absence of arrow from $x_6$ to $x_5$.
\begin{figure}[htbp]
\centering
\subfigure[Ground truth causal relation]{
\includegraphics[width=0.35\textwidth]{figures/ground_truth_causal_relation.eps}
\label{fig:Ground truth causal relation}
}
\quad
\subfigure[transition matrix  of conditional model]{
\includegraphics[width=0.35\textwidth]{figures/causal_relation_conditional.eps}
\label{fig:Causal relation of conditional model}
}
\quad
\subfigure[Causal relation of PC]{
\includegraphics[width=0.35\textwidth]{figures/causal_relation_PC.eps}
\label{fig:Causal relation of PC}
}
\quad
\subfigure[Causal relation of LiNGAM]{
\includegraphics[width=0.35\textwidth]{figures/causal_relation_LiNGAM.eps}
\label{fig:Causal relation of LiNGAM}
}
\caption{Causal relation of different algorithms on Temperature Ozone data}
\end{figure}
\subsection{Recovering causal relation from aggregated time series data}
\label{sec:aggregatedtotal}
In this section, we will apply the adversarial ICA framework to recover causal relation from both synthetic data and real data in aggregating scenario.
\subsubsection{Synthetic data}
Using the same data generated as described in Section \ref{sec:subsampledsynthetic}, low-dimensional observations were obtained by aggregating the high-resolution data using subsampling factork. We set the number of dimensions n= 2,5, aggregating factor k= 2,3,4,5 and samplesize T= 150,300,1000,3000 for aggregating data. We repeat each experiment for 10 times and averaging the results.


Table \ref{table:differentlength_n_2_T_150_300} and Table \ref{table:differentlength_n_2_T_1000_3000} compare the MSE of the estimated parameters $\mathbf{A}$ obtained by models with different length of pieces in aggregating scenario using Algorithm \ref{alg:conditional adversarial learning_aggregated} when the number of dimensions equals to 2 and aggregating factor set to $2,3,4,5$. In Table \ref{table:differentlength_n_2_T_150_300}, the length of observed data is set to 150 and 300 while in Table \ref{table:differentlength_n_2_T_1000_3000} the length of observed data is set to 1000 and 3000. As one compares these two tables, it can be seen that under the same aggregating factor, longer pieces will lead to better results when the total length of observed data increases. When the total length of observed data is fixed, there is a trade-off between the length of each piece and the number of pieces as stated in Section \ref{sec:aggregate}.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{MSE of the recovered transition matrix  esitimated by our divided model with different pieces length on simulated data in aggregating scenario.}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{3}{*}{Pieces length} & \multicolumn{8}{c}{n=2}                                                                                                                                                            \\ \cmidrule(l){2-9} 
                               & \multicolumn{4}{c|}{T=150}                                                                         & \multicolumn{4}{c}{T=300}                                                     \\ \cmidrule(l){2-9} 
                               & k=2               & k=3               & k=4               & \multicolumn{1}{c|}{k=5}               & k=2               & k=3               & k=4               & k=5               \\ \midrule
l=3                            & 7.34e-03          & 1.02e-02          & 5.95e-03          & \multicolumn{1}{c|}{1.23e-02}          & 2.50e-03          & 7.72e-03          & \textbf{5.24e-03} & 1.66e-02          \\ \midrule
l=4                            & \textbf{1.78e-03} & 2.05e-02          & 1.16e-02          & \multicolumn{1}{c|}{1.29e-02}          & 5.48e-03          & 1.35e-02          & 6.69e-03          & 1.66e-02          \\ \midrule
l=5                            & 1.05e-02          & \textbf{8.00e-03} & 1.30e-02          & \multicolumn{1}{c|}{3.59e-02}          & \textbf{1.07e-03} & \textbf{5.87e-03} & 1.00e-02          & 1.67e-02          \\ \midrule
l=6                            & 9.47e-03          & 3.43e-02          & 3.27e-02          & \multicolumn{1}{c|}{3.36e-02}          & 6.12e-03          & 1.79e-02          & 1.07e-02          & \textbf{1.08e-02} \\ \midrule
l=7                            & 5.86e-03          & 1.56e-02          & 2.42e-02          & \multicolumn{1}{c|}{4.12e-02}          & 1.80e-02          & 8.93e-03          & 1.25e-02          & 1.30e-02          \\ \midrule
l=8                            & 1.55e-02          & 1.94e-02          & \textbf{5.28e-03} & \multicolumn{1}{c|}{2.13e-02}          & 9.34e-03          & 7.52e-03          & 9.11e-03          & 1.44e-02          \\ \midrule
l=9                            & 5.70e-03          & 2.28e-02          & 1.19e-02          & \multicolumn{1}{c|}{\textbf{6.11e-02}} & 4.36e-03          & 1.21e-02          & 1.10e-02          & 1.66e-02          \\ \midrule
l=10                           & 4.82e-03          & 9.99e-03          & 8.62e-03          & \multicolumn{1}{c|}{2.52e-02}          & 7.99e-03          & 9.39e-03          & 7.97e-03          & 1.31e-02          \\ \bottomrule
\end{tabular}
    
\label{table:differentlength_n_2_T_150_300}
\end{table}

\begin{table}[]
\centering
\caption{MSE of the recovered transition matrix  esitimated by our divided model with different pieces length on simulated data in aggregating scenario.}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{3}{*}{Pieces length} & \multicolumn{8}{c}{n=2}                                                                                                                                                            \\ \cmidrule(l){2-9} 
                               & \multicolumn{4}{c|}{T=1000}                                                                        & \multicolumn{4}{c}{T=3000}                                                    \\ \cmidrule(l){2-9} 
                               & k=2               & k=3               & k=4               & \multicolumn{1}{c|}{k=5}               & k=2               & k=3               & k=4               & k=5               \\ \midrule
l=3                            & 3.84e-03          & 3.67e-03          & 4.25e-03          & \multicolumn{1}{c|}{2.85e-03}          & 9.16e-04          & 2.59e-03          & 4.82e-03          & 2.36e-03          \\ \midrule
l=4                            & 1.87e-03          & 2.08e-03          & 2.86e-03          & \multicolumn{1}{c|}{2.69e-03}          & 5.27e-04          & 1.57e-03          & 3.43e-03          & 1.87e-03          \\ \midrule
l=5                            & 3.26e-03          & 2.08e-03          & 3.22e-03          & \multicolumn{1}{c|}{2.34e-03}          & 5.15e-04          & 1.39e-03          & 2.90e-03          & 1.34e-03          \\ \midrule
l=6                            & \textbf{1.75e-03} & 2.02e-03          & \textbf{1.87e-03} & \multicolumn{1}{c|}{2.28e-03}          & 6.30e-04          & 9.86e-04          & 2.10e-03          & 7.21e-04          \\ \midrule
l=7                            & 3.27e-03          & 1.80e-03          & 2.85e-03          & \multicolumn{1}{c|}{2.16e-03}          & 3.42e-04          & 9.17e-04          & 1.82e-03          & 6.12e-04          \\ \midrule
l=8                            & 2.91e-03          & 1.73e-03          & 1.94e-03          & \multicolumn{1}{c|}{\textbf{1.26e-03}} & \textbf{2.20e-04} & 7.37e-04          & 1.68e-03          & 5.90e-04          \\ \midrule
l=9                            & 2.19e-03          & \textbf{1.51e-03} & 2.96e-03          & \multicolumn{1}{c|}{1.42e-03}          & 4.85e-04          & 8.20e-04          & 2.03e-03          & 6.66e-04          \\ \midrule
l=10                           & 3.84e-03          & 1.96e-03          & 2.41e-03          & \multicolumn{1}{c|}{1.62e-03}          & 2.94e-04          & \textbf{6.48e-04} & \textbf{1.38e-03} & \textbf{2.99e-04} \\ \bottomrule
\end{tabular}
   
\label{table:differentlength_n_2_T_1000_3000}
\end{table}
In Table \ref{table:aggregatingcompare}, we further compare the results obtained by our divided model(using optimal piece length) with that obtained by the method proposed in \cite{aggregated}. The results are shown for aggregating factors($k=2,3$), length of data($T=150, 300$), and number of dimensions $n=2$. As can be seen from the table, our divided model achieves reasonable results compared with others. CDTA has difficulties dealing with cases where the number of data dimension $n$ and aggregating factor $k$ are larger, while our divided model is able to achieve reasonable results with larger $k$(see Table \ref{table:differentlength_n_2_T_1000_3000} and Table \ref{table:differentlength_n_5_T_1000_3000} when $k>3$) and larger $n$(see Table \ref{table:differentlength_n_5_T_1000_3000} when $n=5$).
\begin{table}[]
\centering
\caption{MSE of the recovered transition matrix  esitimated by different methods on simulated data in aggregating scenario.}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{k=2}                                  & \multicolumn{2}{c}{k=3}             \\ \cmidrule(l){2-5} 
                         & T=150            & \multicolumn{1}{c|}{T=300}            & T=150            & T=300            \\ \midrule
CDTA\_finite             & 2.10e-3          & \multicolumn{1}{c|}{1.19e-3}          & 8.17e-3          & 7.36e-3          \\
CDTA\_Gauss              & 1.28e-2          & \multicolumn{1}{c|}{4.49e-3}          & 1.20e-2          & 7.22e-3          \\
NG-EM                    & 8.75e-2          & \multicolumn{1}{c|}{8.51e-2}          & 5.27e-1          & 1.88e-1          \\
AICA-divided            & \textbf{1.78e-3} & \multicolumn{1}{c|}{\textbf{1.07e-3}} & \textbf{8.00e-3} & \textbf{5.87e-3} \\ \bottomrule
\end{tabular}
    
\label{table:aggregatingcompare}
\end{table}
\begin{table}[]
\centering
\caption{MSE of the recovered transition matrix  esitimated by our divided model with different pieces length on simulated data in aggregating scenario.}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{3}{*}{Pieces length} & \multicolumn{8}{c}{n=5}                                                                                    \\ \cmidrule(l){2-9} 
                               & \multicolumn{4}{c|}{T=1000}                                    & \multicolumn{4}{c}{T=3000}                \\ \cmidrule(l){2-9} 
                               & k=2      & k=3      & k=4      & \multicolumn{1}{c|}{k=5}      & k=2      & k=3      & k=4      & k=5      \\ \midrule
l=3                            & 2.47e-03 & 5.41e-03 & 7.90e-03 & \multicolumn{1}{c|}{1.41e-02} & 5.79e-04 & 9.10e-04 & 3.86e-03 & 2.82e-03 \\ \midrule
l=4                            & 2.52e-03 & 5.05e-03 & 8.82e-03 & \multicolumn{1}{c|}{2.03e-02} & 4.26e-04 & 4.56e-04 & 3.50e-03 & 2.45e-03 \\ \midrule
l=5                            & 1.40e-03 & 8.80e-03 & 1.46e-02 & \multicolumn{1}{c|}{2.56e-02} & 5.58e-04 & 2.12e-03 & 3.69e-03 & 3.19e-03 \\ \midrule
l=6                            & 3.86e-03 & 1.41e-02 & 1.74e-02 & \multicolumn{1}{c|}{3.75e-02} & 3.72e-04 & 1.27e-03 & 3.32e-03 & 4.78e-03 \\ \midrule
l=7                            & 3.03e-03 & 1.29e-02 & 2.58e-02 & \multicolumn{1}{c|}{3.80e-02} & 4.83e-04 & 3.55e-03 & 2.67e-03 & 5.61e-03 \\ \midrule
l=8                            & 4.27e-03 & 1.69e-02 & 6.79e-02 & \multicolumn{1}{c|}{5.00e-02} & 5.55e-04 & 1.51e-03 & 4.51e-03 & 9.87e-03 \\ \midrule
l=9                            & 1.32e-02 & 2.79e-02 & 4.62e-02 & \multicolumn{1}{c|}{4.88e-02} & 5.87e-04 & 5.76e-03 & 1.05e-02 & 1.80e-02 \\ \midrule
l=10                           & 1.78e-02 & 2.06e-02 & 5.42e-02 & \multicolumn{1}{c|}{6.37e-02} & 1.11e-03 & 9.21e-03 & 1.28e-02 & 2.80e-02 \\ \bottomrule
\end{tabular}
    
\label{table:differentlength_n_5_T_1000_3000}
\end{table}
\subsubsection{Real Data}
Using the same Temperature Ozone data, we apply our divided model to recover the causal relation behind data.

Following Section \ref{sec:subsampledrealdata}, we use 50th pair of data to demonstrate the result when $n=2$. The aggregating factor $k$ is set to 2 and pieces length $l$ is set to 3. The estimated transition matrix $\mathbf{A}=\bigl[ \begin{smallmatrix}0.9009 & 0.1709 \\  0.0013 & 0.9796\end{smallmatrix}\bigr]$, from which we can clearly find the causal direction from temperature to ozone.

For case where $n=6$, we use the same method to concatenate the 3 pairs of data. We set aggregating factor $k=2$ and pieces length $l=3$ as well. The estimated transition matrix is
\begin{equation*}
    \mathbf{A} = \left[
    \begin{array}{cccccc}
                            0.6393&  0.8600& -0.0248& -0.0269&  0.0886&  0.0578\\
                            0.0223&  0.4034& -0.0271&  0.0466&  0.0266&  0.0276\\
                            0.0364& -0.0775&  0.5289&  0.8849&  0.0781&  0.0502\\
                           -0.0214&  0.0465&  0.0073&  0.3540& -0.0030&  0.0209\\
                            0.0503& -0.3134&  0.0772&  0.0517&  0.5984& -1.0483\\
                           -0.0483&  0.3691&  0.0339&  0.0031&  0.0215&  0.9123]
    \end{array}\right]
\end{equation*}
We plot the corresponding causal diagram in Figure \ref{fig:causal relation aggregated}. As we can see from the figure, the divided model makes more mistakes compared with Figure \ref{fig:Causal relation of conditional model}. So it can be concluded that the Temperature Ozone data is more likely obtained through subsampling mechanism. 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/causal_relation_aggregated.eps}
    \caption{Causal relation of divided model on Temperature Ozone data}
    \label{fig:causal relation aggregated}
\end{figure}

\subsection{Recovering causal relation from causal model with measurement error}
Table \ref{table:measurementerror} compares the MSE of the causal adjacency matrix estimated by the NG-EM\cite{subsampled} based over-complete ICA method and our AICA method. The synthetic data we used has 5000 data points. We test 4 cases where the number of variables $n$ is 5, 10, 50 and 100 respectively. For each variable, the error term in measurement-error-free causal model\cite{Zhang2018CausalDW} is non-Gaussian distributed, we use Laplace distribution to model the non-Gaussian distribution. The measurement error for each variable is Gaussian distributed with zero mean and variance 0.1. As we can see from the table, AICA perform better then NG-EM when $n=5, 7$. We also compare the time used by the two methods with the same number of iterations. NG-EM is much more time consuming than AICA when $n=5, 7$. When $n>7$($n=50$), NG-EM fails to obtain any results because it uses too much memory, while AICA can still obtain reasonable result. There experiments show that besides the accuracy, AICA uses less time and space than NG-EM as well.

% Since these two methods use different optimization algorithms with different convergence criterion. it's hard to compare their time and space complexity under unified framework. 
\begin{table}[]
    \centering
    \caption{MSE of the recovered causal adjacency matrix by AICA and NG-EM based ICA.}
\begin{tabular}{@{}cccc|ccc@{}}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c|}{MSE}                               & \multicolumn{3}{c}{Time(s)}                        \\ \cmidrule(l){2-7} 
                         & n=5              & n=7              & n=50             & n=5            & n=7            & n=50             \\ \midrule
AICA                     & \textbf{1.04e-3} & \textbf{5.79e-3} & \textbf{1.81e-2} & \textbf{75.01} & \textbf{76.44} & \textbf{1219.34} \\ \midrule
NG-EM                    & 6.98e-3          & 9.85e-3          & -                & 1826.60        & 4032.54        & -                \\ \bottomrule
\end{tabular}
\label{table:measurementerror}
\end{table}

==> v0/intro.tex <==
\emph{Independent component analysis(ICA)} models a \emph{p} observed mixtures over a linear combination of \emph{k} unobserved independent components.
\begin{equation}
\label{equ:ica}
    \mathbf{x}=\mathbf{As}
\end{equation}
where $\mathbf{A} \in \mathds{R}^{p\times k}$, $\mathbf{s}:=(s_1, s_2, ..., s_k)^\top$ and $\mathbf{x}:=(x_1, x_2, ..., x_p)^\top$. $\mathbf{s}$ is a $k$ dimensional latent variable with each dimension called an \emph{independent component}. $\mathbf{x}$ is a $p$ dimensional observed variable with each dimension called a \emph{mixture}. $\mathbf{A}$ is called \emph{mixing matrix}. Given $N$ observations $\mathbf{X}:=(\mathbf{x}_1, \mathbf{x}_2, ..., \mathbf{x}_N)$, we are interested in estimate the mixing matrix $\mathbf{A}$ and corresponding components $\mathbf{S}$.


In standard ICA scenarios, it's normally assumed that 1. At most one component is Gaussian distributed and all the other components must be non-Gaussian distributed; 2. All the components must be mutually independent; 3. The number of components can't exceed that of mixtures(i.e. it requires $p\geq k$). Several algorithms have been proposed to solve the standard ICA problem. \cite{hyvarinen1999fast}, \cite{amari1996new} and \cite{brakel2017learning} try to maximize the independence among the extracted components in different ways. The Central Limit Theorem tells that the distribution of the sum of several independent variables is more likely to be Gaussian. It means that any of two independent random variables is less Gaussian than their sum\cite{hyvarinen2000independent}. Thus, FastICA\cite{hyvarinen1999fast} maximizes the independence of the estimated components by maximizing their non-Gaussianity. Two types of measures of non-Gaussianity are usually used, one is kurtosis and another is negentropy. Besides Gaussianity, Mutual information can also be used as a measure of independence. Mutual information of two variables is zero if and only if they are statistically independent. Thus, \cite{amari1996new} maximizes the independence of the extracted components by minimizing their mutual information. From statistics, we know that two variables are independent if their joint distribution equals to the product of their marginal distributions. Thus \cite{brakel2017learning} maximizing the independence of the components by minimizing the difference between the joint distribution of components and the product of their marginal distributions. Mathematically, minimizing the difference between the joint distribution of components and the product of their marginal distributions can be regarded the same as minimizing the mutual information. So the idea behind \cite{amari1996new} and \cite{brakel2017learning} is almost the same. The difference is the way to implement the idea. Different from the algorithms using independence maximization principle mentioned above, Infomax\cite{pearlmutter1997maximum} uses maximum likelihood principle to solve the ICA problem.

However in over-complete ICA scenarios(i.e. $k \geq p$), the methods used in standard ICA models can not be applied any more. To recover the components and mixing matrix in this case, \cite{hojen2002mean} proposed mean-field ICA(MF-ICA). MF-ICA is a bayesian approach for which we need to specify components distribution and mixing matrix distribution as prior. Then the components can be recovered from the mean of their posterior distribution, and the mixing matrix can be estimated by maximizing a posterior(MAP) solution. Further more, as a probabilistic model, we also need to specify the distribution of the noise covariance as prior. It's usually difficult to specify appropriate prior for the problem, which makes the estimated mixing matrix and components diverse with different priors. In standard ICA, it usually requires an orthonoramlity constraint to be enforced. This constraint makes it difficult to recover components in over-complete ICA. To tackle this problem, \cite{le2011ica} proposes reconstruction ICA(RICA) with a reconstruction loss term added to the loss function to replace the orthonoramlity constraint. The independence maximization principle is also used in RICA. For these independence maximization principle based algorithms, it can't be guaranteed that the recovered components are completely independent. In contrast, our adversarial over-complete ICA framework generates each component from independent noise with a separate network, which guarantees the independence among components.


The contributions of this paper are three fold. First, we propose an adversarial over-complete ICA(AICA) framework, which can be used to estimate the mixing matrix and independent components simultaneously. The independence of the estimated components is guaranteed in this framework. The AICA framework doesn't need further assumption to noise distribution, compared with previous algorithms. Second, we explore the application of the AICA framework in causal discovery. Experiments demonstrate the effectiveness of the framework. that our methods are able to deal with more variables than previous algorithms and obtain better results. Finally, compared with previous causal discovery methods, our method based on AICA framework can deal with more variables.

==> v0/method.tex <==
Here we begin with introducing our method for over-complete ICA problems based on adversarial learning. We can regard $\mathbf{s}$ as multivariate distribution of dimension $k$ and $\mathbf{x}$ as a multivariate distribution of dimension $p$. Thus, $\mathbf{A}$ is a distribution transformer that transform $\mathbf{s}$ to $\mathbf{x}$. Generative adversarial network(GAN)\cite{gan} is an unsupervised generative model that has been proved to have powerful ability of generating vivid samples like natural images, sounds and texts. The principle of GAN is to play a minimax game between a generator and discriminator. The generator maps a particularly distributed noise from it's original space to target space while the discriminator tries to distinguish the samples generated by the generator and real samples. The generator can be regarded as a transformer that transform a noise distribution to target distribution. Thus in ICA, we can use $\hat{\mathbf{A}}$ as a generator $G(\cdot)$ that maps components to mixtures. The mixing matrix $\hat{\mathbf{A}}$ is the parameter of the generator.
\begin{equation}
    \hat{\mathbf{x}} = G_{\hat{\mathbf{A}}}(\hat{\mathbf{s}}) = \hat{\mathbf{A}}\hat{\mathbf{s}}
\end{equation}
Next, we can design a discriminator to discriminate between real samples $\mathbf{x}$ and generated samples $\mathbf{\hat{x}}$. One possible choice for discriminator is multi-layer perceptron(MLP) of which the last layer is sigmoid that outputs probability. Another possible choice is distance measurement between different distributions, such as KL divergence or kernel maximum mean discrepancy(MMD)\cite{MMD}. \cite{mmdgan} combines neural networks and MMD by first mapping the samples from original space to another space using neural networks such as MLP or CNN, then the MMD is used to measure the distance between distributions in the new space through the mapped samples. 
In ICA scenarios, the components have to be non-Gaussian distributed instead of Gaussian. So we further use multi-layer perceptron(MLP) to learn a mapping function $f(\cdot)$ that transform any random noise $\mathbf{z}$ to corresponding components. For example, we can model $\mathbf{z}$ as Gaussian noise and $\hat{\mathbf{s}}$ as mixture of Gaussian.
\begin{equation}
    \hat{\mathbf{s}} = f_{\theta}(\mathbf{z})
\end{equation}
The parameters $\theta$ of the mapping function $f(\cdot)$ can be learned end to end in this adversarial over-complete ICA framework. The optimization goal for the framework can be formulated as following
\begin{equation}
\label{equ:opt}
    \argmin \limits_{\hat{\mathbf{A}}, \theta}M(\mathds{P}(\mathbf{x}), \mathds{P}(G_{\hat{\mathbf{A}}}(f_\theta(\mathbf{z})))
\end{equation}
where $M$ is MMD distance measurement function. See Figure \ref{fig:over-completeica} for graphical illustration for the generator of the adversarial over-complete ICA framework with 4 components and 3 mixtures. While most of the previous algorithms for both under-complete scenario(\cite{hyvarinen1999fast}, \cite{brakel2017learning}, \cite{amari1996new}, \cite{hyvarinen2000independent}) and over-complete scenario(\cite{le2011ica}, \cite{hojen2002mean}) try to maximize the independence among the recovered components, the components recovered by our adversarial ICA algorithm is essentially independent because each component is generated by an individual MLP from independent noise. It can be seen from  Figure \ref{fig:over-completeica}.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/overcomplete_ica.eps}
    \caption{Graphical illustration for the generator of the adversarial over-complete ICA framework. $\mathbf{z}_1, \mathbf{z}_2, \mathbf{z}_3, \mathbf{z}_4$ is i.i.d Gaussian noise, each MLP is initialized with different values because we require all the components(dimensions) of $\hat{\mathbf{s}}=[\hat{s}_1, \hat{s}_2, \hat{s}_3, \hat{s}_4]$ to be mutually independent.}
    \label{fig:over-completeica}
\end{figure}


The remaining problem is the identifiability of the over-complete ICA model. Luckily, it has been proved in \cite{identifiabilityofica} that under the following assumptions, the mixing matrix $\mathbf{A}$ can be estimated up to the permutation and scaling indeterminacies(including the sign indeterminacy) of the columns. And the components can also be estimated under these assumptions. 


\textbf{Assumption 1.} All components are non-Gaussian distributed with non-vanishing characteristic functions.

\textbf{Assumption 2.} Rank[$\mathbf{A} \odot \mathbf{A}$] = $k$, where $k$ is the number of components.

When the identifiabilit of the model is satisfied, the solution for the model is unique. Thus we can use optimization method such as SGD to solve Equation \ref{equ:opt}.

The general adversarial over-complete ICA framework can be concluded in Algorithm \ref{alg:ica framework}. In Section \ref{sec:experiment}, we will compare the result of our adversarial ICA algorithm with those of previous over-complete ICA algorithms(\cite{hojen2002mean}, \cite{le2011ica}). The experiment demonstrates the effectiveness of our algorithms over others.

\begin{algorithm}[t]
\caption{General Adversarial over-complete ICA Framework(AICA)} 
\label{alg:ica framework}
\begin{algorithmic}[1]
    \State Get a minibatch of samples from $p(\mathbf{z})$ 
    \State Mapping $\mathbf{z}$ using parameterized $f_\theta(\cdot)$ into domain of components, get $\mathbf{\Hat{s}}$
    \State Multiply $\mathbf{\Hat{s}}$ by mixing matrix $\hat{\mathbf{A}}$, get mixtures $\mathbf{\Hat{x}}$
    \State Get a minibatch of samples from $p(\mathbf{x})$ 
    \State Calculate distribution distance between $p(\mathbf{\Hat{x}})$ and $p(\mathbf{x})$ using MMD $M(\mathds{P}(x), \mathds{P}(G_{\hat{A}}(f_\theta(z)))$
    \State Using optimization algorithms such as SGD to update $\hat{\mathbf{A}}$ and $\theta$ by minimizing MMD
    \State Repeat step 1 to step 6 until max iterations reached
\end{algorithmic}
\end{algorithm}

==> v1/application.tex <==
\subsection{Causal Discovery under Measurement Error}
Measurement error (\eg noise caused by sensors) in the observed data can lead to inaccurate result of various causal discovery methods. Recently, it was proven that the causal relation is identifiable from data with measurement error under linearity non-Gaussian noise assumptions \cite{Zhang2018CausalDW}. Based on the identifiability theory in \cite{Zhang2018CausalDW}, we propose a causal discovery algorithm by extending LFOICA with additional constraints.

Following \cite{Zhang2018CausalDW}, we use the LiNGAM model \cite{shimizu2006linear} to represent the causal relations on the data without measurement error. More specifically, the causal model is $\tilde{\mathbf{X}}=\mathbf{B} \tilde{\mathbf{X}}+\tilde{\mathbf{E}}$, where $\tilde{\mathbf{X}}$ is the data generated by causal model without measurement error, $\tilde{\mathbf{E}}$ is independent non-Gaussian noise terms, and $\mathbf{B}$ is the corresponding causal adjacency matrix in which $B_{ij}$ is the coefficient of the direct causal influence from $\tilde{X}_j$ to $\tilde{X}_i$ and $B_{ii}=0$ (no self-influence). In fact, $\tilde{\mathbf{X}}$ is a linear transformation of the noise term $\tilde{\mathbf{E}}$ because the linear model can be re-expressed by $\tilde{\mathbf{X}}=(\mathbf{I}-\mathbf{B})^{-1} \tilde{\mathbf{E}}$. Then, the model with with measurement error $\mathbf{E}$ can be obtained by
\begin{align}
\label{equ:measurementerror}
     \mathbf{X} = \tilde{\mathbf{X}} + \mathbf{E}&=(\mathbf{I}-\mathbf{B})^{-1} \tilde{\mathbf{E}} +\mathbf{E}
    =\left[(\mathbf{I}-\mathbf{B})^{-1}\quad \mathbf{I}\right]\left[\begin{array}{c}
         \tilde{\mathbf{E}}\\
         \mathbf{E}
    \end{array}\right],
\end{align}
where $\mathbf{X}$ is observed data, $\mathbf{E}$ is measurement error. Obviously,  (\ref{equ:measurementerror}) is a special OCIA model with  $\left[(\mathbf{I}-\mathbf{B})^{-1}\quad \mathbf{I}\right]$ as the mixing matrix. Therefore, we can readily extend our LFOICA algorithm to estimate the causal adjacency matrix $\mathbf{B}$.

\subsection{Causal Discovery from Low-Resolution Time Series}
Granger causal analysis has been shown sensitive to temporal resolution/frequency of time series. If the temporal resolution is lower than the underlying causal resolution, it is generally difficult to discover the high-resolution causal relations. Recently, it has been shown that the high-resolution causal relation is identifiable from low-resolution time series under the linearity and non-Gaussian assumptions \cite{subsampled,aggregated}. The corresponding models can also be viewed as extensions of OICA and the model parameters are estimated in the Expectation Maximization framework with variational inference or sampling to approximate the posterior distribution of ICs \cite{subsampled,aggregated}. However, these algorithms are either inaccurate or computationally expensive. To make causal discovery from low-resolution time series practically feasible, we further extend our LFOICA to discover causal relations from such data.




Following \cite{subsampled}, we assume the data at original causal frequency as a first-order vector autoregressive process (VAR(1)):
\begin{equation}
\label{equ:originalprocess}
    \mathbf{x}_t=\mathbf{A}\mathbf{x}_{t-1}+\mathbf{e}_t,
\end{equation}
where $\mathbf{x}_t\in \mathbb{R}^{n}$ is the high frequency data and $\mathbf{e}_t \in \mathbb{R}^{n}$ represents independent non-Gaussian noise in the causal system. $\mathbf{A} \in \mathbb{R}^{n\times n}$ is the causal transition matrix at true causal frequency with $A_{ij}$ representing the temporal causal influence from variable $j$ to variable $i$. The corresponding   low-resolution (\ie down-sampled) data \cite{subsampled}. As done in \cite{subsampled,aggregated}, we consider two schemes under which the low frequency data can be obtained. One is ``subsampling'': for every $k$ consecutive data points, one is kept and the others being dropped. The other is ``aggregating'': the average of $k$ consecutive and non-overlapping data points is taken as the new observation. We will detail our algorithms to address these two types of problems one by one.

\paragraph{Causal Discovery from Subsampled Time Series}
\label{sec:subsample}
We consider the following subsampling scheme with subsampling factor $k$. 
\begin{align} 
\label{equ:subsample}
\tilde{\mathbf{x}}_{t+1}=\mathbf{A}^k\mathbf{\tilde{x}}_t+\mathbf{L\tilde{e}}_{t+1}
\end{align}
Where $\tilde{\mathbf{x}}$ is the observed data subsampled from $\mathbf{x}$, $\mathbf{L}= [\mathbf{I, A, A^2, ..., A^{k-1}}], \mathbf{\tilde{e}} = (\mathbf{e}_{1+tk-0}^\intercal, \mathbf{e}_{1+tk-1}^\intercal, ..., \mathbf{e}_{1+tk-(k-1)}^\intercal)^\intercal \notag$.  We are interested in estimating the transition matrix $\mathbf{A}$ from the subsampled data.
(\ref{equ:subsample}) can be regarded as a VAR(1) model with noise $\mathbf{\tilde{e}}$ that is independent among different time steps as well. Graphical representation of this subsampled data is illustrated in Figure \ref{fig:subsamplingk}. 
% \begin{figure}[htbp]
% \centering 
% \includegraphics[width=0.45\textwidth]{figures/subsampled.eps}
% \caption{Graphical representation of subsampled data with sampling factor $k$}
% \label{fig:subsampledprocess}
% \end{figure}

Basically, \cite{subsampled} makes use of second-order statistical information (\ie autocovariances) to first estimate $\mathbf{A}^k$ and get rid of the contribution of the first term in the right handside of (\ref{equ:subsample}) to give $   \Delta{\tilde{\mathbf{x}}}_{t+1} = \mathbf{L\tilde{e}}_{t+1}$, where $\Delta{\tilde{\mathbf{x}}}_{t+1}=\tilde{\mathbf{x}}_{t+1}-\mathbf{A}^k\mathbf{\tilde{x}}_t$. It can be easily seen that this equation has the same OICA form as (\ref{equ:ica}). The LFOICA framework can be applied to learn the transition matrix $\mathbf{A}$. However, the estimation of $\mathbf{A}^k$ may be inaccurate as the number of variables grows larger. This will lead to incorrect estimation of $\mathbf{A}$. Conditional GAN \cite{cgan} uses training labels as additional inputs to both generator and discriminator. Motivated by this, we modify the LFOICA framework to have conditional input. We call this modified model as LFOICA-conditional. See Figure \ref{fig:conditionalsubsampled} for graphical representation for this LFOICA-conditional model. Detailed description about LFOICA-conditional algorithm can be found in section 3 of Supplementary Material. This model learns the relation between $\mathbf{\tilde{e}}_t$ and $\mathbf{\tilde{x}}_t$ (\ie $\mathbf{L}$) and the relation between $\mathbf{\tilde{x}}_t$ and  $\mathbf{\tilde{x}}_{t+1}$ (\ie $\mathbf{A}^k$) jointly, without explicit estimation of $\mathbf{A}^k$. % Suppose we have $N$ subsampled data $(\mathbf{\tilde{x}}_1, \mathbf{\tilde{x}}_2, ..., \mathbf{\tilde{x}}_N)$. We first sample $\mathbf{\tilde{x}}_t$ from the subsampled data as conditions. Then we take $\mathbf{\tilde{x}}_{t+1}$ as target data. The generator takes both non-Gaussian noise and conditions as inputs and generate $\mathbf{\hat{\tilde{x}}}_{t+1}$. $\mathbf{\hat{\tilde{x}}}_{t+1}$ at different time steps can be regarded as independent by condition on $\mathbf{\tilde{x}}_{t}$. Then MMD can be calculated as the distance between the conditional distributions $p(\mathbf{\tilde{x}}_{t+1}|\mathbf{\tilde{x}}_{t})$ and $p(\mathbf{\hat{\tilde{x}}}_{t+1}|\mathbf{\tilde{x}}_{t})$. Finally optimization method is used to minimize MMD. 

% \begin{figure}[htbp]
% \centering 
% \subfigure[Baseline model]{
% \label{fig:baselinesubsampled}
% \includegraphics[width=0.45\textwidth]{figures/baseline_model.eps}}
% \subfigure[Conditional model]{
% \label{fig:conditionalsubsampled}
% \includegraphics[width=0.45\textwidth]{figures/conditional_model.eps}}
% \caption{Graphical representations of two models for subsampled data with sampling factor $k$}
% \end{figure}

It has been proved in \cite{subsampled} that besides the assumptions needed for the identifiability of OICA, if we further assume that the $n$ components of $\mathbf{e}_{t}$ in (\ref{equ:originalprocess}) have different distributions, the permutation and scaling indeterminacies can be eliminated with only sign indeterminacy left.

% The AICA-conditional model achieves desirable result on subsampled time series data, which is demonstrated in Section \ref{sec:subsampledtotal}.

\paragraph{Causal Discovery from Aggregated Time Series}
\label{sec:aggregate}
We consider the following aggregating scheme with aggregating factor $k$. Detailed derivation can be found in \cite{aggregated}.
\begin{align}
\label{equ:aggregate}
\notag \tilde{\mathbf{x}}_{t}&=\mathbf{A}^{k}\tilde{\mathbf{x}}_{t-1}+\left[\mathbf{I} \quad \sum_{l=0}^{1} \mathbf{A}^{l} \quad \cdots \quad \sum_{l=0}^{k-1} \quad \mathbf{A}^{l}\sum_{l=1}^{k-1} \mathbf{A}^{l} \quad \ldots \quad \sum_{i=k-2}^{k-1} \mathbf{A}^{l} \quad \mathbf{A}^{k-1} \right] \left[ \begin{array}{c}{\tilde{\mathbf{e}}_{t}^{(0)}} \\ {\tilde{\mathbf{e}}_{t}^{(1)}} \\ {\vdots} \\ {\tilde{\mathbf{e}}_{t}^{(2 k-2)}}\end{array}\right]\\
&=\mathbf{A}^{k} \tilde{\mathbf{x}}_{t-1}+\mathbf{H} \tilde{\mathbf{e}}_{t}
% \mathbf{A}^{k} \tilde{\mathbf{x}}_{t-1}+\mathbf{M}_{0} \mathbf{\epsilon}_{t}+\mathbf{M}_{1} \mathbf{\epsilon}_{t-1} 
\end{align}
% Where
% \begin{align*}
%     \left[ \begin{array}{c}{\widetilde{\mathbf{e}}_{t}^{(0)}} \\ {\tilde{\mathbf{e}}_{t}^{(1)}} \\ {\widetilde{\mathbf{e}}_{t}^{(1)}} \\ {\vdots} \\ {\widetilde{\mathbf{e}}_{t}^{(2 k-2)}}\end{array}\right]=\mathbf{F} \left[ \begin{array}{c}{\widetilde{\mathbf{e}}_{t-1}^{(0)}} \\ {\tilde{\mathbf{e}}_{t-1}^{(1)}} \\ {\widetilde{\mathbf{e}}_{t-1}^{(1)}} \\ {\vdots} \\ {\widetilde{\mathbf{e}}_{t-1}^{(2 k-2)}}\end{array}\right]+\left[ \begin{array}{c}{\mathbf{e}_{t k}} \\ {\mathbf{e}_{t k-1}} \\ {\vdots} \\ {\mathbf{e}_{(t-1) k+1}} \\ {\mathbf{O}_{(n k-n) \times 1}}\end{array}\right],
%     \mathbf{F}=\left[ \begin{array}{cc}{\mathbf{0}_{n k \times(n k-n)}} & {\mathbf{0}_{n k \times(n k)}} \\ {\mathbf{I}_{(n k-n) \times(n k-n)}} & {\mathbf{0}_{(n k-n) \times(n k)}}\end{array}\right]
% \end{align*}
% $\tilde{\mathbf{e}}_{t}^{(l)}=\mathbf{e}_{t k-l}$.
Different from subsampling process, the noise term in (\ref{equ:aggregate}) is dependent at different time steps (detailed explanation can be found in section 4 of Supplementary Material). Graphical representation for aggregated data as a special state space model is illustrated in Figure \ref{fig:aggregatedprocess}. \cite{graphicalGAN} proposes State Space GAN (SSGAN) as an instance of graphical GAN to learn recognition model and generation model jointly. Inspired by SSGAN and it's application to Moving MNIST \cite{movingmnist}, we process our aggregated time series data to mimic the special traits of Moving MNIST, in which each data point is a time sequence. We divide the aggregated time series into pieces of equal length without overlapping. Figure \ref{fig:pieces} is an illustration of one such piece of length 4, with $\tilde{\mathbf{x}}_t$ as a conditional term.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/conditional_model_aggregated_piece.eps}
%     \caption{Graphical illustration of divided piece of aggregated time series with length 4}
%     \label{fig:pieces}
% \end{figure}

We can consider our aggregated data as composed of many such pieces without overlapping. Based on the idea of SSGAN, generation model and inference (recognition) model are learned jointly by matching the joint distribution $q(\hat{\tilde{\mathbf{e}}}_{t+1}, \hat{\tilde{\mathbf{e}}}_{t+2}, \hat{\tilde{\mathbf{e}}}_{t+3}, \hat{\tilde{\mathbf{x}}}_{t+1}, \hat{\tilde{\mathbf{x}}}_{t+2}, \hat{\tilde{\mathbf{x}}}_{t+3})$ and $p(\tilde{\mathbf{e}}_{t+1}, \tilde{\mathbf{e}}_{t+2}, \tilde{\mathbf{e}}_{t+3}, \tilde{\mathbf{x}}_{t+1}, \tilde{\mathbf{x}}_{t+2}, \tilde{\mathbf{x}}_{t+3})$, where $q$ and $p$ represent distributions generated by recognition model and generation model respectively. While in this problem, it's unnecessary to do inference because we don't care about latent variables $\tilde{\mathbf{e}}$. So we simply match $p(\hat{\tilde{\mathbf{x}}}_{t+1}, \hat{\tilde{\mathbf{x}}}_{t+2}, \hat{\tilde{\mathbf{x}}}_{t+3}|\tilde{\mathbf{x}}_{t})$ and $p(\tilde{\mathbf{x}}_{t+1}, \tilde{\mathbf{x}}_{t+2}, \tilde{\mathbf{x}}_{t+3}|\tilde{\mathbf{x}}_{t})$ with conditional input $\tilde{\mathbf{x}}_{t}$. As the pieces are non-overlapping, the dependence issue is avoided because all the pieces can be regarded as independent. It's obvious that longer pieces are better because they model longer relations. However, in practice the number of observed data points (size of dataset) is limited, which means the total length of aggregated time series is limited. Longer pieces will lead to smaller number of pieces, which means the batch size is smaller. And small batch size will lead to inaccurate result when calculating MMD \cite{gmmn}. There is a trade off between the length of each piece and the number of pieces. We call this method as LFOICA-divided. The effects of different length of piece and detailed description of LFOICA-divided can be found in section 4 of Supplementary Material.
% Detailed description is illustrated in Algorithm \ref{alg:conditional adversarial learning_aggregated}.
\begin{figure}[htbp]
    \centering
    \subfigure[]{
\label{fig:subsamplingk}
\includegraphics[width=0.35\textwidth]{figures/subsampled.eps}}
\subfigure[]{
\label{fig:conditionalsubsampled}
\includegraphics[width=0.35\textwidth]{figures/conditional_model.eps}}
\subfigure[]{
\label{fig:aggregatedprocess}
\includegraphics[width=0.35\textwidth]{figures/aggregated_v2.eps}}
\subfigure[]{
\label{fig:pieces}
\includegraphics[width=0.35\textwidth]{figures/conditional_model_aggregated_piece_v2.eps}}
\caption{(a) subsampled data with subsampling factor $k$. (b) LFOICA-conditional model for subsampled data. (c) aggregated data with aggregating factor $k$. (d) a divided piece with length 4 used in LFOICA-divided model for aggregated data.}
\end{figure}

% \begin{algorithm}[htbp]
% \caption{LFOICA For Aggregated Data(LFOICA-divided)} 
% \label{alg:conditional adversarial learning_aggregated}
% \begin{algorithmic}[1]
%     \State Divide the aggregated time series into pieces of length $l$. Select a minibatch from the pieces.
%     \State Take the first element in each piece as condition and the other elements as targets. Taking Figure \ref{fig:pieces} as an example, $\tilde{\mathbf{x}}_t$ is the condition and $\tilde{\mathbf{x}}_{t+1},\tilde{\mathbf{x}}_{t+2},\tilde{\mathbf{x}}_{t+3}$ are targets.
%     \State Get a minibatch of samples from $p(\mathbf{z})$.
%     \State Mapping each sample $\mathbf{z}$ using parameterized mapping $f_\theta(\cdot)$, get non-Gaussian noise(For example, $\hat{\tilde{\mathbf{e}}}_{t+1},\hat{\tilde{\mathbf{e}}}_{t+2},\hat{\tilde{\mathbf{e}}}_{t+3}$ in Figure \ref{fig:pieces}). All the noises are i.i.d.
%     \State Generator takes the noise generated in the previous step and condition $\tilde{\mathbf{x}}_t$ as inputs and generate target data $\hat{\mathbf{\tilde{x}}}_{t+1}$ using Equation \ref{equ:aggregate}, $\hat{\tilde{\mathbf{x}}}_{t+2}, \hat{\tilde{\mathbf{x}}}_{t+3}, ..., \hat{\tilde{\mathbf{x}}}_{t+n-1}$ are generated in the same way.
%     \State Calculate distribution distance between $q(\hat{\tilde{\mathbf{x}}}_{t+1}, \hat{\tilde{\mathbf{x}}}_{t+2}, ..., \hat{\tilde{\mathbf{x}}}_{t+n-1}|\tilde{\mathbf{x}}_{t})$ and $p(\tilde{\mathbf{x}}_{t+1}, \tilde{\mathbf{x}}_{t+2}, ..., \tilde{\mathbf{x}}_{t+n-1}|\tilde{\mathbf{x}}_{t})$ using MMD. Update $\mathbf{A}$ and $\theta$ by minimizing MMD.
%     \State Repeat step 1 to step 6 until max iterations reached.
% \end{algorithmic}
% \end{algorithm}

==> v1/experiment.tex <==
We first compare the results obtained by LFOICA and several OICA algorithms on synthetic OICA data. Then we apply LFOICA framework in two causal discovery problems using both synthetic and real data. All the experiments are conducted on a workstation with one i9-9900X CPU and two GeForce RTX 2080Ti GPUs.
\subsection{Recovering Mixing Matrix Using Synthetic OICA Data}
In this section, we compare LFOICA with several well-known OICA algorithms on synthetic data. Experiment details including data generation and ways to eliminate the permutation and scaling indeterminacies for comparison can be found in Section 1.1 and 1.2 of the Supplementary Material.

In Table \ref{table:overcompleteica}, RICA represents reconstruction ICA \cite{le2011ica}, MFICA\_Gauss and MFICA\_MoG represents mean-field ICA \cite{hojen2002mean} with the prior distribution of ICs set as Gaussian and mixture of Gaussian respectively. NG-EM represents the EM based ICA \cite{subsampled}. $p$ is the number of mixtures, $d$ is the number of ICs. For each algorithm, we conduct experiments in 4 cases ([p=2 d=4], [p=3 d=6], [p=4 d=8] and [p=5 d=10]). We compare the mean square error (MSE) between the estimated mixing matrix and the ground-truth mixing matrix used to generate the data. Each experiment is repeated 10 times and the results are averaged. As we can see, our LFOICA achieves best result compared with the others. We also compare the recovered components using LFOICA with the ground-truth, the result can be found in Section 1.3 of the Supplementary Material.

\begin{table}[]
\centering
\caption{MSE of the recovered mixing matrix by different methods on synthetic OICA data.}
\begin{tabular}{@{}ccccc@{}}
\toprule
Methods        & p=2, d=4         & p=3, d=6         & p=4, d=8         & p=5, d=10        \\ \midrule
RICA           & 2.26e-2          & 1.54e-2          & 9.03e-3          & 7.54e-3          \\
MFICA\_Gauss   & 4.54e-2          & 2.45e-2          & 4.21e-2          & 3.18e-2          \\
MFICA\_MoG     & 2.38e-2          & 9.17e-3          & 2.43e-2          & 1.04e-2          \\
NG-EM & 1.82e-2          & 6.56e-3          & 1.21e-2          & 6.34e-3          \\
LFOICA           & \textbf{4.61e-3} & \textbf{5.95e-3} & \textbf{6.96e-3} & \textbf{5.92e-3} \\ \bottomrule
\end{tabular}
 
\label{table:overcompleteica}
\end{table}

\subsection{Recovering Causal Relation from Causal Model with Measurement Error}
\paragraph{Synthetic Data}
Details about how the data is generated can be found in section 2.1 of Supplementary Material. Table \ref{table:measurementerror} compares the MSE between the ground-truth causal adjacency matrix and that estimated by NG-EM \cite{subsampled} and our LFOICA. The synthetic data we used contains 5000 data points. We test 3 cases where the number of variables $n$ is 5, 10, 50 respectively.
% For each variable, the error term in measurement-error-free causal model \cite{Zhang2018CausalDW} is non-Gaussian distributed, we use Laplace distribution to model the non-Gaussian distribution. The measurement error for each variable is Gaussian distributed with zero mean and variance 0.1.
As we can see from the table, LFOICA performs better then NG-EM. We also compare the time used by the two methods with the same number of iterations. As can be seen, NG-EM is much more time consuming than LFOICA (because EM needs to calculate the posterior). When $n>7$ ($n=50$), NG-EM fails to obtain any results because it runs out of memory, while LFOICA can still obtain reasonable result. These experiments show that besides the efficacy, LFOICA is computationally more efficient and use less space than NG-EM as well.
\paragraph{Real Data}
We apply LFOICA to Sachs’s data \cite{sachs2005causal} with 11 variables. Sachs's data is a record of various cellular protein concentrations under a variety of exogenous chemical inputs, which can be regarded as a causal model with measurement error. The estimated causal adjacency matrix by LFOICA can be found in section 2.2 of Supplementary Material. Here we visualize the causal diagram estimated by LFOICA and the ground-truth in Figure \ref{fig:LFOICA diagram} and \ref{fig:gt diagram}. As a comparison, we further visualize the causal diagram estimated by generalized LiNGAM (LiNG) \cite{lacerda2012discovering} and the ground-truth in Figure \ref{fig:lingam diagram } and \ref{fig:gt diagram lingam}. As we can see, LiNG fails to recover most of the causal directions while LFOICA performs better. This experiment makes an important point: measurement error can lead to inaccurate result of various causal discovery algorithms, while LFOICA can be applied to causal model under measurement error with better results.
\begin{figure}[htbp]
\centering 
\subfigure[]{
\label{fig:LFOICA diagram}
\includegraphics[width=0.23\textwidth]{figures/LFOICA_sachs_color.eps}}
\subfigure[]{
\label{fig:gt diagram}
\includegraphics[width=0.23\textwidth]{figures/GT_sachs_color.eps}}
\subfigure[]{
\label{fig:lingam diagram }
\includegraphics[width=0.23\textwidth]{figures/lingam_sachs_color.eps}}
\subfigure[]{
\label{fig:gt diagram lingam}
\includegraphics[width=0.23\textwidth]{figures/GT_sachs_color_lingam.eps}}
\caption{(a)(b) Causal diagram by LFOICA and ground-truth. (c)(d) Causal diagram by LiNG and Ground-truth. The red arrows in (a) and (b) are redundant and missing causal directions of LFOICA compared with ground-truth.  The red arrows in (c) and (d) are redundant and missing causal directions of LiNG compared with ground-truth. The blue arrows in (a) and (c) are converse causal directions of LFOICA and LiNG respectively compared with ground-truth.}
\end{figure}

% \begin{figure}[htbp]
% \centering 
% \subfigure[Causal diagram by LiNGAM]{
% \label{fig:lingam diagram }
% \includegraphics[width=0.33\textwidth]{figures/lingam_sachs_color.eps}}
% \subfigure[Ground-truth causal diagram]{
% \label{fig:gt diagram lingam}
% \includegraphics[width=0.33\textwidth]{figures/GT_sachs_color_lingam.eps}}
% \caption{The red arrows in (a) are the redundant causal directions. The red arrows in (b) are the missing causal directions. The blue arrows in (a) are the converse causal directions.}
% \end{figure}
% Since these two methods use different optimization algorithms with different convergence criterion. it's hard to compare their time and space complexity under unified framework. 
\begin{table}[]
    \centering
    \caption{MSE of the recovered causal adjacency matrix by LFOICA and NG-EM.}
\begin{tabular}{@{}cccc|ccc@{}}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c|}{MSE}                               & \multicolumn{3}{c}{Time(s)}                        \\ \cmidrule(l){2-7} 
                         & n=5              & n=7              & n=50             & n=5            & n=7            & n=50             \\ \midrule
LFOICA                     & \textbf{1.04e-3} & \textbf{5.79e-3} & \textbf{1.81e-2} & \textbf{75.01} & \textbf{76.44} & \textbf{1219.34} \\ \midrule
NG-EM                    & 6.98e-3          & 9.85e-3          & -                & 1826.60        & 4032.54        & -                \\ \bottomrule
\end{tabular}
\label{table:measurementerror}
\end{table}

\subsection{Recovering Causal Relation from Low-Resolution Time Series Data}
\label{sec:subsampledtotal}
% We apply LFOICA here to recover causal relation from synthetic subsampled data and real data.
\paragraph{Synthetic Data}
% \label{sec:subsampledsynthetic}
Following \cite{subsampled}, we generate the synthetic time series data at the original causal frequency using VAR(1) model described by (\ref{equ:originalprocess}). Details about how the data is generated can be found in section 3.1 of the Supplementary Material. Table \ref{table:subsampledcompare_n_2_1} shows the MSE between the ground-truth transition matrix and that estimated by different algorithms when number of variables $n=2$. We conduct experiments when the subsampling factor $k=2,3,4,5$ and size of dataset $T=100, 300$. Each experiment is repeated 10 times and the results are averaged. As one can see from Table \ref{table:subsampledcompare_n_2_1}, LFOICA-conditional achieves comparable result as NG-EM and NG-MF \cite{subsampled}. NG-EM has better performance when the number of data points is small ($T=100$) probably because the MMD distance measure used in LFOICA-conditional may be inaccurate with small number of samples. When the number of data points is larger ($T=300$), LFOICA-conditional obtains best results. We also conduct experiment when $n$ is larger ($n=5$). The result can be found in Section 3.2 of the Supplementary Material.
\begin{table}[]
\centering
\caption{MSE of the recovered transition matrix by different methods on synthetic subsampled data.}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{3}{*}{Methods} & \multicolumn{8}{c}{n=2}                                                                                                                                                    \\ \cmidrule(l){2-9} 
                         & \multicolumn{4}{c|}{T=100}                                                                     & \multicolumn{4}{c}{T=300}                                                 \\ \cmidrule(l){2-9} 
                         & k=2              & k=3              & k=4              & \multicolumn{1}{c|}{k=5}              & k=2              & k=3              & k=4              & k=5              \\ \midrule
LFOICA-conditional         & 7.25e-3          & 7.88e-3          & \textbf{8.45e-3} & \multicolumn{1}{c|}{\textbf{9.00e-3}} & \textbf{1.12e-3} & \textbf{3.87e-3} & \textbf{4.07e-3} & \textbf{6.23e-3} \\ \midrule
NG-EM                    & \textbf{6.50e-3} & \textbf{7.32e-3} & 1.02e-2          & \multicolumn{1}{c|}{1.04e-2}          & 7.24e-3          & 9.11e-3          & 9.54e-3          & 9.98e-3          \\ \midrule
NG-MF                    & 9.09e-3          & 9.89e-3          & 1.24e-2          & \multicolumn{1}{c|}{2.19e-2}                               & 8.46e-3          & 8.76e-3          & 1.01e-2          & 2.20e-2          \\ \bottomrule
\end{tabular}
    
\label{table:subsampledcompare_n_2_1}
\end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \multirow{3}{*}{Methods} & \multicolumn{8}{c}{n=2}                                                                            \\ \cmidrule(l){2-9} 
%                          & \multicolumn{4}{c|}{T=1000}                                & \multicolumn{4}{c}{T=3000}            \\ \cmidrule(l){2-9} 
%                          & k=2     & k=3     & k=4     & \multicolumn{1}{c|}{k=5}     & k=2     & k=3     & k=4     & k=5     \\ \midrule
% Baseline model           & 6.76e-4 & 7.95e-5 & 4.20e-4 & \multicolumn{1}{c|}{1.11e-3} & 8.22e-5 & 1.38e-4 & 6.58e-5 & 2.72e-4 \\ \midrule
% Conditional model        & 1.06e-3 & 2.94e-4 & 3.88e-4 & \multicolumn{1}{c|}{9.54e-4} & 2.28e-4 & 1.68e-4 & 1.90e-4 & 9.60e-4 \\ \midrule
% Other methods            & -       & -       & -       & \multicolumn{1}{c|}{-}       & -       & -       & -       & -       \\ \bottomrule
% \end{tabular}
%     
% \caption{MSE of the recovered causal relation by different methods on simulated data in subsampling scenario. The results are shown for subsampling factors$(k=2, 3, 4, 5)$, length of data $(T=1000, 3000)$ and number of dimensions $n=5$. Here \textit{Other methods} includes methods NG-EM, NG-MF and G-EM proposed in \cite{subsampled}, method BFL proposed in \cite{boot1967further} and method SW proposed in \cite{stram1986methodological}.}
% \label{table:subsampledcompare_n_2_2}
% \end{table}


% Table \ref{table:subsampledcompare_n_5_1} and Table \ref{table:subsampledcompare_n_5_2} shows the mean square error (MSE) of the estimated parameters $\mathbf{A}$ when number of dimensions $n=5$ in subsampling scenario. As one can see from Table \ref{table:subsampledcompare_n_5_1} and Table \ref{table:subsampledcompare_n_5_2}, although both baseline model and condition model are desirable enough to recover the original causal relation $\mathbf{A}$, the conditional model obtains better result that that of baseline model. One instance of original causal relation $\mathbf{A}$ and the estimated counterpart is recorded as follows, whose MSE is $5.5\times 10^{-3}$. It shows that $\tilde{\mathbf{A}}$ is very close to $\mathbf{A}$ under this MSE.
% \begin{equation*}
% \mathbf{A}=
% \left[
% \begin{array}{ccccc}
%      0.78 & 0.02 & 0.05 & 0.03 & 0.06 \\
%      0.18 & 0.89 & 0 & 0.05 & -0.03 \\
%      0.08 & 0.01 & 0.36 & 0 & -0.04 \\
%      0 & 0 & 0.11 & 0.79 & -0.03 \\
%      0 & 0.01 & 0.01 & 0.02 & 0.66
% \end{array}
% \right]
% , \tilde{\mathbf{A}}=
% \left[
% \begin{array}{ccccc}
%     0.7684 &  0.0137&  0.1033&  0.0046&  0.0541 \\
%     0.1734&  0.8847&  0.0327&  0.0248& -0.0259 \\
%     0.0959& -0.0008&  0.2999&  0.0019& -0.0395 \\
%     0.0120& -0.0076&  0.0816&  0.8054& -0.0332 \\
%     -0.0005& -0.0257& -0.3104&  0.2003&  0.7156 \\
% \end{array}
% \right]
% \end{equation*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


% \begin{table}[]
% \centering
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
% \multirow{3}{*}{Methods} & \multicolumn{8}{c}{n=5}                                                                            \\ \cmidrule(l){2-9} 
%                          & \multicolumn{4}{c|}{T=1000}                                & \multicolumn{4}{c}{T=3000}            \\ \cmidrule(l){2-9} 
%                          & k=2     & k=3     & k=4     & \multicolumn{1}{c|}{k=5}     & k=2     & k=3     & k=4     & k=5     \\ \midrule
% Baseline model           & 5.42e-3 & 4.74e-3 & 4.11e-3 & \multicolumn{1}{c|}{3.25e-3} & 4.38e-3 & 6.78e-4 & 1.66e-3 & 5.33e-4 \\ \midrule
% Conditional model        & 5.00e-4 & 1.73e-3 & 4.08e-3 & \multicolumn{1}{c|}{3.94e-3} & 1.89e-4 & 2e-4    & 3.77e-4 & 1.17e-4 \\ \midrule
% Other methods            & -       & -       & -       & \multicolumn{1}{c|}{-}       & -       & -       & -       & -       \\ \bottomrule
% \end{tabular}
%     
% \caption{MSE of the recovered causal relation by different methods on simulated data in subsampling scenario. The results are shown for subsampling factors$(k=2, 3, 4, 5)$, length of data $(T=1000, 3000)$ and number of dimensions $n=5$.}
% \label{table:subsampledcompare_n_5_2}
% \end{table}
\paragraph{Real Data}
% \label{sec:subsampledrealdata}
Here we use \href{https://webdav.tuebingen.mpg.de/cause-effect/}{Temperature Ozone Data} \cite{JMLR:v17:14-518}, which corresponds to 49th, 50th and 51st causal-effect pairs in the database. These three temperature ozone pairs are taken at three different places in 2009. Each pair of data contains two variables, ozone and temperature with the ground-truth causal direction temperature $\longrightarrow$ ozone. To demonstrate the result when $n=2$, we use 50th pair as in \cite{subsampled}. The optimal subsampling factor $k$ can be determined using the method of cross-validation on the log-likelihood of the models. Here we use $k=2$ according to \cite{subsampled}. The estimated transition matrix $\mathbf{A}=\bigl[ \begin{smallmatrix}0.9310 & 0.1295 \\  -0.0017 & 0.9996\end{smallmatrix}\bigr]$ (the first variable is ozone and the second is temperature in the matrix). from which we can clearly find the causal direction from temperature to ozone. We also conduct experiments when $n=6$. The result can be found in section 3.3 in Supplementary Material.
\subsection{Recovering Causal Relation from Aggregated Time Series Data}
\label{sec:aggregatedtotal}
% We apply LFOICA here to recover causal relation from synthetic aggregated data and real data.
\paragraph{Synthetic Data}
Using the same data generating process as described in Section \ref{sec:subsampledtotal}, we then down-sample the data with different aggregating factors. The effects of different pieces length are compared, which can be found in section 4.2 of the Supplementary Material. In Table \ref{table:aggregatingcompare}, we compare the LFOICA-divided (using optimal pieces length) with CDTA \cite{aggregated} and NG-EM. The results are shown for $k=2,3$, $T=150, 300$, and $n=2$. As can be seen from the table, LFOICA-divided achieves best results compared with others.
\begin{table}[]
\centering
\caption{MSE of the recovered transition matrix by different methods on synthetic aggregated data.}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{k=2}                                  & \multicolumn{2}{c}{k=3}             \\ \cmidrule(l){2-5} 
                         & T=150            & \multicolumn{1}{c|}{T=300}            & T=150            & T=300            \\ \midrule
CDTA\_finite             & 2.10e-3          & \multicolumn{1}{c|}{1.19e-3}          & 8.17e-3          & 7.36e-3          \\
CDTA\_Gauss              & 1.28e-2          & \multicolumn{1}{c|}{4.49e-3}          & 1.20e-2          & 7.22e-3          \\
NG-EM                    & 8.75e-2          & \multicolumn{1}{c|}{8.51e-2}          & 5.27e-1          & 1.88e-1          \\
LFOICA-divided            & \textbf{1.78e-3} & \multicolumn{1}{c|}{\textbf{1.07e-3}} & \textbf{8.00e-3} & \textbf{5.87e-3} \\ \bottomrule
\end{tabular}
\label{table:aggregatingcompare}
\end{table}
\paragraph{Real Data}
We apply LFOICA-divided to recover the causal relation using the same Temperature Ozone Data. Following \cite{aggregated}, we set $n=2$, $k=2$, and optimal pieces length is set to $l=3$. The estimated transition matrix $\mathbf{A}=\bigl[ \begin{smallmatrix}0.9009 & 0.1709 \\  0.0013 & 0.9796\end{smallmatrix}\bigr]$, from which we can clearly find the causal direction from temperature to ozone. We also conduct experiments when $n=6$. The result can be found in section 4.3 in Supplementary Material.

==> v1/intro.tex <==
Discovering causal relations among variables has been an important problem in various fields such as medical science and social science. Because conducting randomized controlled trials is usually expensive or infeasible, discovering causal relations from observational data, \ie causal discovery\cite{Pearl:2000:CMR:331969,spirtes2000causation}) has received much attention in the past decades. The classical causal discovery methods can be roughly categorized into constraint-based methods, such as PC \cite{spirtes2000causation} and FCI \cite{spirtes2000causation}, and score-based methods such as GES \cite{chickering2002optimal}. However, these methods output multiple causal graphs in the Markov equivalence classes. Since the seminal work \cite{shimizu2006linear}, there have been various methods that have complete identifiability of the causal model by making use of constrained Functional Causal Models (FCMs) (\cite{shimizu2006linear,hoyer2009nonlinear,zhang2009identifiability}). For example, with linearity and non-Gaussian noise constraints, it was shown that the causal model
is identifiable from data with measurement noise \cite{Zhang2018CausalDW} or missing values \cite{hoyer2008estimation,geiger2015causal,subsampled,aggregated,subsample_tank}.

Recently, some causal discovery algorithms  (\cite{shimizu2006linear}, \cite{zhang2009identifiability}, \cite{hoyer2009nonlinear}) based on Functional Causal Models (FCMs) were proposed with the ability to distinguish between different Directed Acyclic Graphs (DAGs) in the same equivalence class\cite{glymour2019review}, which is known as identifiability. The identifiability gives the credit to non-Gaussian assumption on the noise distribution in causal models. 
% with the identifiability of the model under specific assumptions(\cite{Zhang2018CausalDW}, \cite{subsampled}, \cite{aggregated}, \cite{shimizu2006linear}).

The algorithms mentioned above(\cite{shimizu2006linear}, \cite{zhang2009identifiability}, \cite{hoyer2009nonlinear}) make the strong assumption of no latent confounders. With the assumption of no confounders, some algorithms based on FCMs such as \cite{shimizu2006linear} and \cite{zhang2009identifiability} resort to undercomplete ICA. Typical undercomplete ICA algorithms(\cite{hyvarinen1999fast}, \cite{amari1996new}, \cite{brakel2017learning}) base on the idea of maximizing the independence of the recovered components. \cite{hyvarinen1999fast} maximize the independence by maximizing non-Gaussianity while \cite{amari1996new} and \cite{brakel2017learning} maximize the independence by minimizing the mutual information or the distance between the joint distribution of recovered components and the product of their marginal distributions. However, The no latent confounders assumption is not acceptable because confounders always exist in empirical science. \cite{hoyer2008estimation} take latent confounders into consideration in the LiNGAM framework. Model with latent variables can be expressed in the form OICA. The fundamental problem in OICA is to decompose $p$ mixtures into $d$ independent components, where $d>p$. Typical OICA algorithms such as mean-field ICA\cite{hojen2002mean} and EM based ICA (NG-EM\cite{subsampled}) make strong parametric assumptions to the density function of the independent components, which restrict their applications to real word data. NG-EM is computationally expensive due to the inference of posterior distribution of independent components, especially when the number of variables is large. Additional noises are assumed in NG-EM, which lead to it's slow convergence. To tackle these problems, we propose likelihood-free overcomplete ICA (LFOICA). LFOICA avoids any parametric assumptions to density function by using neural networks to learn the distribution of independent components implicitly. By minimize the distribution distance between the generated mixtures from LFOICA model and mixtures from the observed data, all the parameters including the mixing matrix in LFOICA model can be optimized via backpropagation (BP) and stochastic gradient descent (SGD). Benefit from BP and SGD, our LFOICA algorithm can scale to cases with large number of variables.

% To demonstrate the effectiveness of our method, we apply LFOICA in two causal discovery problem. One is causal discovery under measurement error, the other is causal discovery from down-sampled time series data.

The contributions of this paper are three fold. First, we propose an likelihood-free overcomplete ICA (LFOICA) framework, which can be used to estimate the mixing matrix and independent components simultaneously. Given properly designed structures, LFOICA can model any distributions of independent components without parametric assumptions. It's computational efficient compared with previous algorithms. Second, we explore the application of LFOICA in causal discovery with measurement error. Experiments demonstrate the efficacy of the framework. Finally, we adapt LFOICA to causal discovery from down-sampled time series. Two down-sampling scenarios are considered and LFOICA works well for both scenarios.

==> v1/method.tex <==
\subsection{General framework}
Typical ICA problem can be expressed using
\begin{equation}
\label{equ:ica}
    \mathbf{x} = \mathbf{As}
\end{equation}
where $\mathbf{x}\in \mathds{R}^{p}, \mathbf{s}\in \mathds{R}^{d}, \mathbf{A}\in \mathds{R}^{p\times d}$ are known as mixtures, independent components and mixing matrix respectively. The target is to recover $\mathbf{A}$ and $\mathbf{s}$ from observed mixtures $\mathbf{x}$. 

The generator in GAN\cite{gan} can be regarded as a transformer that transform random noise from noise domain to target domain. Motivated by this, we use a generator $G(\cdot)$ that transforms components to mixtures linearly using $\hat{\mathbf{x}} = G_{\hat{\mathbf{A}}}(\hat{\mathbf{s}}) = \hat{\mathbf{A}}\hat{\mathbf{s}}$ in ICA. $\hat{\mathbf{A}}$ is the parameter of the generator. According to GAN's architecture, when the discriminator is optimal, the target for the generator is to minimize the distribution distance between the generated samples and true samples. Many distance measurements for distributions can be used, such as KL divergence\cite{gan}, Wasserstein distance\cite{arjovsky2017wasserstein} and kernel maximum mean discrepancy(MMD)\cite{MMD}. We use MMD in this paper with the generator $G_{\hat{\mathbf{A}}}$ trying to minimize MMD between the observed mixtures $\mathbf{x}$ and generated mixtures $\mathbf{\hat{x}}$ by optimizing $\hat{\mathbf{A}}$.
% Following GAN's architecture, a discriminator is needed to discriminate between observed mixtures $\mathbf{x}$ and generated mixtures $\mathbf{\hat{x}}$. Many distance measurements for distributions can be used as discriminator, such as KL divergence\cite{gan}, Wasserstein distance\cite{arjovsky2017wasserstein} or kernel maximum mean discrepancy(MMD)\cite{MMD}. 

In ICA scenario, the components have to be independently non-Gaussian distributed. So we further use multi-layer perceptron(MLP) to learn a mapping function $f(\cdot)$ that transform any noise distribution $\mathbf{z}$ to corresponding components distributions using $    \hat{\mathbf{s}} = f_{\theta}(\mathbf{z})
$. We model $\mathbf{z}:=(z_1, z_2, ..., z_d)^\top$ as independent Gaussian noise in this paper.

The parameters $\theta$ of the mapping function $f(\cdot)$ and the mixing matrix $\hat{\mathbf{A}}$ in the generator can be learned end to end in this framework using \ref{equ:opt}.
\begin{align}
\label{equ:opt}
    \hat{\mathbf{A}}^*, \theta^*=\argmin \limits_{\hat{\mathbf{A}}, \theta}M\left(\mathds{P}(\mathbf{x}\right), \mathds{P}(G_{\hat{\mathbf{A}}}(f_\theta(\mathbf{z}))) + \lambda \left\| \hat{\mathbf{A}}\right\|_1
\end{align}
Here $M(\cdot)$ in \ref{equ:opt} is MMD distance measurement function
\begin{align*}
    M(\mathds{P}(\mathbf{x}), \mathds{P}(\mathbf{y})) = \left\|\frac{1}{N} \sum_{i=1}^{N} \phi\left(x_{i}\right)-\frac{1}{M} \sum_{j=1}^{M} \phi\left(y_{j}\right)\right\|^{2}
\end{align*}
Choosing $\phi$ to be identify function will lead to match the mean, and other choices of $\phi$ can be used to match higher order moments\cite{li2015generative}. Kernel trick such as Gaussian kernel can be applied here to match arbitrary order moment.

We illustrate the generating process of the LFOICA framework with 4 components and 3 mixtures in Figure \ref{fig:overcompleteica}. While most of the previous algorithms for both undercomplete scenario \cite{hyvarinen1999fast, brakel2017learning, amari1996new, hyvarinen2000independent} and overcomplete scenario \cite{le2011ica} try to maximize the independence among the recovered components, the components recovered by our LFOICA is essentially independent because the noise $\mathbf{z}_i$ for each component $\mathbf{s}_i$ is independently sampled and each component is generated by a separate MLP from the independent noise, as can be seen in the figure.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/overcomplete_ica.eps}
    \caption{Generator of the LFOICA framework. $\mathbf{z}_1, \mathbf{z}_2, \mathbf{z}_3, \mathbf{z}_4$ is i.i.d Gaussian noise.}
    \label{fig:overcompleteica}
\end{figure}

Next problem is the identifiability of the OICA model. It has been proved that under some assumptions including the non-Gaussian assumption, the mixing matrix $\mathbf{A}$ can be estimated up to permutation and scaling indeterminacies(including the sign indeterminacy) of the columns\cite{identifiabilityofica}. The assumptions and proof for the identifiability can be found in \cite{identifiabilityofica}.

General LFOICA framework is concluded in Algorithm \ref{alg:ica framework}. In Section \ref{sec:experiment}, we will compare LFOICA with several overcomplete ICA algorithms \cite{hojen2002mean, le2011ica}. Experiment demonstrates the effectiveness of our algorithms over others.

\begin{algorithm}[t]
\caption{General Likelihood-Free Overcomplete ICA Framework(LFOICA)} 
\label{alg:ica framework}
\begin{algorithmic}[1]
    \State Get a minibatch of samples from noise distribution $p(\mathbf{z})$.
    \State Mapping $\mathbf{z}$ using parameterized $f_\theta(\cdot)$ from noise domain into components domain, get $\mathbf{\Hat{s}}$.
    \State Generate mixtures $\mathbf{\Hat{x}}=\hat{\mathbf{A}}\mathbf{\Hat{s}}$.
    \State Get a minibatch of samples from the distribution of observed mixtures $p(\mathbf{x})$.
    \State update $\hat{\mathbf{A}}$ and $\theta$ by minimizing distance between $p(\mathbf{\Hat{x}})$ and $p(\mathbf{x})$ using \ref{equ:opt}.
    % \State Using optimization algorithms such as SGD to update $\hat{\mathbf{A}}$ and $\theta$ by minimizing MMD.
    \State Repeat step 1 to step 5 until max iterations reached.
\end{algorithmic}
\end{algorithm}

\subsection{Two practical issues}
We further consider two issues when apply the LFOICA framewrok into practical problems.

\paragraph{Sparsity}
Based on the fact that the mixing matrix is sparse in many practical applications, we use LASSO regularizer, which corresponds to the second term in \ref{equ:opt}. However, the LASSO regularizer is suboptimal due to it's non-smoothness, which may cause gradient issue in back-propagation. To avoid this issue, we introduce proximal gradient method\cite{Moolekamp2018}. The proximal mapping for LASSO regularizer corresponds to the soft-thresholding operator.
\begin{equation*}
   \operatorname{prox}_{\gamma}(\hat{\mathbf{A}})=S_{\lambda \gamma}(\hat{\mathbf{A}})=\left\{\begin{array}{ll}{\hat{\mathbf{A}}-\lambda \gamma} & {\text { if } \hat{\mathbf{A}}>\lambda \gamma} \\ {0} & {\text { if }-\lambda \gamma \leq \hat{\mathbf{A}} \leq \lambda \gamma} \\ {\hat{\mathbf{A}}+\lambda \gamma} & {\text { if } \hat{\mathbf{A}}<-\lambda \gamma}\end{array}\right.
\end{equation*}
this operator is then applied to the gradient descent step. Here $\lambda, \gamma$ are regularization coefficient and learning rate respectively.
\begin{equation*}
    \hat{\mathbf{A}}^{(t)}=\operatorname{prox}_{\gamma_{t}}\left(\hat{\mathbf{A}}^{(t-1)}-\gamma_{t} \nabla M_{\hat{\mathbf{A}}}\left(\cdot\right)\right), \quad t=1,2,3, \ldots
\end{equation*}

\paragraph{Insufficient data}
Sufficient data is necessary if we want to successfully learn the large amount of parameters in the MLPs. However, sometimes it's hard to obtain enough data. In this case we use Gaussian mixtures instead of MLPs to model the non-Gaussian distribution of independent components
\begin{equation*}
    p_{\hat{s}_{i}}=\sum_{z_{i}=1}^{m} w_{i, z_{i}} \mathcal{N}\left(\hat{s}_{i} | \mu_{i, z_{i}}, \sigma_{i, z_{i}}^{2}\right), \quad i=1,2, \ldots, d
\end{equation*}
Where $m$ is the number of Gaussian components for each Gaussian mixture. $d$ is the number of independent components. However, unlike MLPs, the operations of sampling from Gaussian distribution and categorical distribution in Gaussian mixing process are not differentiable. To tackle this problem, we introduce two reparameterization tricks. According to \cite{kingma2013auto}, we can sample from $\mathcal{N}(\mu_{i, z_{i}}, \sigma_{i, z_{i}}^{2})$ by first sampling from $\epsilon \sim \mathcal{N}(0, 1)$, then computing $\mu_{i, z_{i}}+ \epsilon \sigma_{i, z_{i}}$. In this way, the gradient can be back-propagated to $\mu_{i, z_{i}}$ and $\sigma_{i, z_{i}}$ successfully. Then we use the second reparameterization trick, which is also known as Gumbel softmax trick\cite{jang2016categorical}. We can sample from categorical distribution by first sampling gumbel noise $g_{z_i}=-\log \left(-\log \left(u_{z_i}\right)\right), u_{z_i} \sim Uniform(0,1)$, then computing $\frac{\exp \left(\frac{\log \left(w_{z_i}\right)+g_{z_i}}{\tau}\right)}{\sum_{z_j=1}^{m} \exp \left(\frac{\log \left(w_{z_j}\right)+g_{z_j}}{\tau}\right)}$. In this way, the gradient can be back-propagated to $w_{z_j}$ successfully.




